Research Artifacts in Software Engineering Publications: Status and Trends

The Software Engineering (SE) community has been embracing the open science policy and encouraging researchers to disclose artifacts in their publications. However, the status and trends of artifact practice and quality remain unclear, lacking insights on further improvement. In this paper, we present an empirical study to characterize the research artifacts in SE publications. Specifically, we manually collect 1,487 artifacts from all 2,196 papers published in top-tier SE conferences (ASE, FSE, ICSE, and ISSTA) from 2017 to 2022. We investigate the common practices (e.g., URL location and format, storage websites), maintenance activities (e.g., last update time and URL validity), popularity (e.g., the number of stars on GitHub and characteristics), and quality (e.g., documentation and code smell) of these artifacts. Based on our analysis, we reveal a rise in publications providing artifacts. The usage of Zenodo for sharing artifacts has significantly increased. However, artifacts stored in GitHub tend to receive few stars, indicating a limited influence on real-world SE applications. We summarize the results and provide suggestions to different stakeholders in conjunction with current guidelines.

==> deprecated/IEEE-old/sections_abandoned/RQ2.tex <==

\subsection{RQ2 Quality}
RQ2 characterizes the quality of artefacts from three aspects: documentation, tests for code and code smell. In the field of software engineering, these three characteristics are important indicators of project quality and code quality.
\subsubsection{RQ2.1 Documentation}
Because the artefacts are completely unfamiliar to readers, a detailed readme document is a must. Artefacts without readme documents are so difficult for users to check, install and use that they cannot guarantee the reproducibility. Therefore, RQ2.1 focuses on the situation of documentation of artefacts.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/2-1/Figure_6.png}
\end{center}
\caption{The number of the artefacts with and without readme documents.}
\label{documentation}
\end{figure}

As shown in Figure \ref{documentation}, 96.5\% of artefacts have readme documents, and only 3.5\% of artefacts are without any document. In fact, the artefacts without any document are usually less popular, as \draft{number\%} of \draft{number} artefacts without documentation only have few than \draft{3} stars.

\textbf{Finding 6}: 
The readme documents help users understand, install and use artefacts. The readme documents of artefacts are highly valued because 96.5\% of artefacts have readme documents.

\subsubsection{RQ2.2 Tests}
Testing is an integral part of software engineering. Any software needs to be tested before it is released to minimize potential bugs, and the same is true for artefacts. Writing tests for the code in artefacts can make artefacts more robust and ensure users to use artefacts smoothly. Therefore, RQ2.2 explores whether there are tests written for the code in the artefacts.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/2-1/Figure_7.png}
\end{center}
\caption{The number of the artefacts with and without tests written for their code.\jie{revise, detaileds suggestions in wechat group}}
\label{testcode}
\end{figure}

From the statistical results of the past five years, \draft{number} of the artefacts have files of tests. For the artefacts that focus on processing data, there are relatively few tests in artefacts. Only \draft{number} of them have constructed lightweight test tools to test whether the current environment is suitable, such as whether GPU support can be obtained. And there are \draft{number} of artefacts which develop tools contain tests. \draft{If there are other kinds of artefacts that have tests, we also need to point out here.}\He{the analysis here for processing data or developing tools is not very accurate, perhaps focusing on the linking between language and test tools will be more scientific}

\textbf{Finding 7}: Although the importance of testing has become a consensus in software engineering field, only  23.7\%,  of artefacts have tests written for the code. Artefacts without being tested cannot guarantee robustness, and users may encounter more potential bugs when using these artefacts, resulting in irreproducibility. Therefore, writing tests for code should be emphasized in the construction of future artefacts.

\subsubsection{RQ2.3 Code Smell}
To explore the code quality of artefacts, RQ2.3 detects the code smell of artefacts. As mentioned in section \uppercase\expandafter{\romannumeral3}, because Python and Java are the two most commonly used programming languages in artefacts and they are the only two programming languages to be used by more than \draft{10} artefacts each year from 2017 to 2021 at a usage ratio of over 10\%, we only detect the code smell of Python and Java for the convenience of comparative analysis. 

\textbf{Python Code Quality}. After obtaining the Python artefacts that meet our requirements mentioned in section \uppercase\expandafter{\romannumeral3}, we detect the code quality of Python in these artefacts by Pylint. In addition, noted that during the detecting process of Pylint, \draft{number} artefacts cannot be analyzed due to various errors. The errors are often caused by the proportion of Python code is too small or various different code files are mixed. So we remove these repositories that cannot be analysed and generate code quality reports. Finally, \draft{number} of \draft{number} artefacts were successfully detected from 2017 to 2021. Over \draft{number\%} repositories can be detected successfully, so our code quality detection results can reflect the general code quality situation of Python artefacts.

In order to investigate the overall code quality situation of the artefacts from 2017 to 2021, we have statistics for five aspects of the Python code quality and calculate the average number of each kind of messages per artefact per year. Figure \ref{plot-python-smell} shows the average number of five kinds of messages per artefact detected by Pylint from 2017 to 2021. The number of Convention Messages per year is the largest compared to other messages. In 2020, there are 1457 Convention Messages on average in each repository using python, and the repositories in 2021 are basically the same. The number of Warning Messages accounts for the second largest number and its number decrease significantly in 2021. The Error Messages, Reflector Messages, and Information Messages accounts for the remaining \draft{number\%}. 
In detail, Convention Messages and Warning Messages are usually caused by some non-standard programming behavior. Too many Convention Messages means that the code style of artefacts do not get enough attention.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/2-4/plot-python-smell.png}
\end{center}
\caption{\draft{need to be updated! }The number of Code Quality Message of Python from 2017 to 2021.}
\label{plot-python-smell}
\end{figure}

Further more, we want to explore whether there are some common children messages of code quality problem in artefacts. Therefore, we count the top three most children messages among each kind of messages and checked the reasons for these children messages in detail, as shown in Table \ref{pythoncodequalitycount}.

\begin{table}[htbp]
\caption{Pylint's messages with top3 proportion}
The Table shows the messages with top 3 proportion given by Pylint from 2019 to 2021.\draft{need to be updated and add Table description!}
\begin{center}
\begin{tabular}{c|c|c|c}
Year&ID&Meaning&Percentage(\%)\\
\hline
2017&E0401&import-error&27\\
 &E0001&syntax-error&27\\
 &E0602&undefined-variable&26\\
\cline{2-4}
 &W0311&bad-indentation&56\\
 &W0109&duplicate-key&7\\
 &W0611&unused-import&4\\
\cline{2-4}
 &C0301&line-too-long&98\\
 &C0103&invalid-name&1\\
 &C0116&missing-function-docstring&1\\
\cline{2-4}
 &R0801&duplicate-code&82\\
 &R1725&super-with-arguments&3\\
 &R1732&consider-using-with&2\\
\hline
2018&E0602&undefined-variable&46\\
 &E0401&import-error&37\\
 &E0001&syntax-error&7\\
\cline{2-4}
 &W0311&bad-indentation&67\\
 &W0621&redefined-outer-name&6\\
 &W0611&unused-import&5\\
\cline{2-4}
 &C0103&invalid-name&33\\
 &C0116&missing-function-docstring&19\\
 &C0301&line-too-long&11\\
\cline{2-4}
 &R0801&duplicate-code&18\\
 &R1705&no-else-return&10\\
 &R0914&too-many-locals&10\\
\cline{2-4}
 &I1101&c-extension-no-member&100\\
\hline
2019&E0401&import-error&48\\
 &E0602&undefined-variable&26\\
 &E1101&no-member&9\\
\cline{2-4}
 &W0311&bad-indentation&85\\
 &W0611&unused-import&2\\
 &W0612&unused-variable&2\\
\cline{2-4}
 &C0103&invalid-name&54\\
 &C0116&missing-function-docstring&15\\
 &C0301&line-too-long&10\\
\cline{2-4}
 &R1705&no-else-return&16\\
 &R0914&too-many-locals&9\\
 &R0903&too-few-public-methods&8\\
\hline
2020&E0602&undefined-variable&35\\
 &E0601&used-before-assignment&27\\
 &E0401&import-error&25\\
\cline{2-4}
 &W0311&bad-indentation&41\\
 &W0612&unused-variable&14\\
 &W1406&redundant-u-string-prefix&8\\
\cline{2-4}
 &C0103&invalid-name&49\\
 &C0116&missing-function-docstring&16\\
 &C0301&line-too-long&15\\
\cline{2-4}
 &R0801&duplicate-code&23\\
 &R1732&consider-using-with&10\\
 &R0913&too-many-arguments&9\\
\cline{2-4}
 &I1101&c-extension-no-member&100\\
\hline
2021&E0602&undefined-variable&46\\
 &E0401&import-error&37\\
 &E1101&no-member&8\\
\cline{2-4}
 &W0311&bad-indentation&44\\
 &W0614&unused-wildcard-import&15\\
 &W0611&unused-import&8\\
\cline{2-4}
 &C0103&invalid-name&40\\
 &C0301&line-too-long&16\\
 &C0116&missing-function-docstring&10\\
\cline{2-4}
 &R0801&duplicate-code&32\\
 &R0914&too-many-locals&9\\
 &R1732&consider-using-with&7\\
\cline{2-4}
 &I1101&c-extension-no-member&100\\

\end{tabular}
\label{pythoncodequalitycount}
\end{center}
\end{table}

For Convention Message, invalid-name is a prominent problem. This message appears when the name doesn't conform to naming rules associated to its type (constant, variable, class...). Since Convention Message has the largest number of all five types of messages and invalid-name accounts for the largest proportion of Convention Message, it can be considered that most researchers do not pay attention to the naming requirements of different data types. What's more, missing-function-docstring and line-too-long are also two common Convention Messages, which ranking second and third in Convention Messages in 2019 and 2020, respectively. Lack of comments for functions and overly long lines of code might make it difficult for users to read and use the replication code. Therefore, researchers should pay more attention to these three issues when programming with python.

Warning Message is the message type with the second highest proportion of warehouse messages. Among them, bad-indentation occupies a very high proportion, 85\% in 2019, 41\% in 2020 and 7\% in 2021, especially in 2019 and 2020, the number of which is the largest in Warning Messages, is the generation of Warning messages. The main reason for the Message. In Python code, indentation represents the difference between code blocks. Small changes in indentation can lead to huge differences in program behavior. Therefore, it is a problem worthy of attention. Fortunately, the proportion of bad-indentation has decreased year by year, indicating that the code quality in this area has improved. In addition to bad-indentation, unused variable is also a type of Warning Message that often appears.

Import-errors accounted for 48\%, 25\% and 23\% of Error Messages in the past three years respectively. At the same time, undefined-variable and no-member also occupy a larger number in 2019 and 2020 as prominent problems. In fact, Error Message often means that the code is very likely to have bugs. Therefore, when writing the code of the replication package, researchers should pay attention to the three problems of [import error, undefined-variable and no member].

Refactor Message mainly guides how to better refactor the code. Messages of this type are relatively scattered, and the highest proportion in three years is no more than 30\%, which reflects that the code warehouse does not have too concentrated and prominent problems in this regard. But it is worth noting that there are also some sub-types of Message that often appear, such as duplicate-code, too-many-locals, no-else-return, etc. Paying attention to these issues in the subsequent artifact development process can make the code structure clearer and the code more concise and readable.

The overall number of Information Messages is very small, and the main problem is that member variables that do not exist in the C extension are accessed. In fact, pylint's documentation gives a description of this subtype of message, Due to unavailability of source static analysis is impossible, but it may be performed by introspecting living objects in run-time.

\textbf{Finding 8}: 1) The number of python code artefacts has increased in the past five years with similar code quality. 
2) There are no fatal problems or too much error messages in artefacts. And convention and warning problems account for a large proportion of \draft{number\%} and \draft{number\%} in 2021 respectively. 
3) Import-error, undefined-variable, no-member, bad-indentation, unused-variable, invalid-name, missing-function-docstring, line-too-long, duplicate-code, too-many-locals, a total of 10 problems are common. In order to make the code of artifacts more robust and readable, researchers should pay special attention to these problem in the future development of the Python artefacts.

\draft{If not enough, we can still add some analysis about the code smell distribution of repositories in each year, to see whether the number of repositories with good code smell has grown during past 3 years.}

\textbf{Java Code Smell}.
After obtaining the Java artefacts that use Java and meet our requirements, we detected their code smell of Java using PMD. On the purpose of exploring the overall code smell situation of Java in artefacts, we counted the detection results of PMD and calculated the average numbers of various code smells in artefacts, which are shown in Figure \ref{plot-java-smell}. In general, the problems of code smell in the two aspects of Code Style and Documentation occupy a large proportion of \draft{number\%}. The number of Code Style problems accounted for the most in 2019, reduced in 2020, and increased slightly in 2021. Documentation problems increased significantly in 2021 compared to 2020. In addition, the types and corresponding quantities of Java code smells have not changed much in the past five years. This reflects the ongoing lack of attention to Code Style and Documentation.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/2-4/plot-java-smell.png}
\end{center}
\caption{The number of Code Smell of Java from 2017 to 2021.}
\label{plot-java-smell}
\end{figure}

In order to further explore the code smell of Java artefacts, we counted the proportion of children code smells among each code smell type. By doing so, whether there are common problems in the Java artefacts can be found out. Similar to Python, we selected the top three children code smells among each code smell type, and calculated the proportion of them in the corresponding code smell type. Table \ref{javacodesmellcount} shows the statistical results.

In the Best Practice category, JUnitAssertionsShouldIncludeMessage and SystemPrintln are the top two issues in 2019-2021, with collections accounting for more than 33\% and 50\% in 2019. This shows that these two problems are easily overlooked by researchers when developing Java projects.

In the Code Style category, the three subtypes LocalVariableCouldBeFinal, MethodArgumentCouldBeFinal, and ShortVariable occupied the top three in the three years. Among them, the first two subtypes account for a little more than the third subtype, accounting for more than 20\% each year. These data show that these three Code Smell subtypes have always been relatively easy to appear in the java code development of artifact.

In terms of the total number, Documentation is a relatively prominent Code Smell in the java warehouse in the past three years, so we focus on analyzing the key code smell subtypes that exist in this area. Table \ref{javacodesmellcount} shows that CommentRequired is the most common Code smell, accounting for more than 74\% in three years. Followed by CommentSize, accounting for more than 22\% in three years. These two code smell subtypes together account for more than 95\% of the total number of Documentation types, and are the most prominent and worthy of attention.

\textbf{Finding 9:} 1) In the past five years, the number of Java artefacts has decreased with similar types and quantity distributions of code smells and many common problems. 2) The two code smells of Code Style and Documentation account for a large proportion of over \draft{number\%} in total. 3) There are three children code smells of LocalVariableCouldBeFinal, MethodArgumentCouldBeFinal, and ShortVariable under Code Style, two children code smells of CommentRequired and CommentSize under Documentation, and LawOfDemeter subtype under Design, and two children code smells of BeanMembersShouldSerialize and AvoidLiteralsInIfCondition under Error Prone, three children code smells of AvoidSynchronizedAtMethodLevel, UseConcurrentHashMap, and DoNotUseThreads under Multithreading, and three children code smells of AvoidInstantiatingObjectsInLoops, RedundantFieldInitializer, and ConsecutiveAppendsShouldReuse under Performance are all common problems in Java artefacts. These 
code smells are so common that researchers can focus more on them in future contruction of Java artefacts, making the code of artifact more robust and readable.

\begin{tcolorbox}
\textbf{\underline{Answer to RQ2:}} 
The documentation gets lots of attention while tests for code don't. 96.5\% of artefacts have readme documents while less than 23.7\% of artefacts have tests written for their code. Conventional code style and documentation are two most overlooked code smells of artefacts of no matter Python or Java. For Python, \draft{\%} and \draft{\%} of code quality problems are Convention Messages and Documentation Messages. For Java, Code Style and Documentation account for \draft{\%} and \draft{\%} respectively. What's more, as shown in Finding 8 and 9, there are many common code smell problems in artifacts in past five years.
\end{tcolorbox}

% In the past three years, the number of python code repositories has increased significantly, and the number of java code repositories has decreased slightly, but the average number of code smells that are prone to occur in each repository and their corresponding proportions have not changed much. Whether in python repositories or java repositories, code style and comment documentation are the two biggest issues. It can be said that in terms of the code quality of the artifact, the code smells that appear have a high commonality. Therefore, no matter what language is used, in order to improve the code quality and ensure that readers can understand and reproduce, software engineering researchers can pay more attention to the compliance with the agreed code specification and write enough code comments according to the comment specification.

\begin{table*}[htbp]
\caption{PMD's messages with top3 proportion}
The Table shows the messages with top 3 proportion given by PMD from 2019 to 2021.
\begin{center}
\begin{tabular}{c|c|c|c}

Year & Ruleset & Rule & Percentage(\%)\\
\hline
2017&Best Practices&SystemPrintln&19\\
 & &UnusedLocalVariable&10\\
 & &JUnitAssertionsShouldIncludeMessage&9\\
\cline{2-4}
 &Code Style&LocalVariableCouldBeFinal&23\\
 & &MethodArgumentCouldBeFinal&21\\
 & &ShortVariable&11\\
\cline{2-4}
 &Design&LawOfDemeter&72\\
 & &CyclomaticComplexity&3\\
 & &AvoidThrowingRawExceptionTypes&3\\
\cline{2-4}
 &Documentation&CommentRequired&64\\
 & &CommentSize&34\\
 & &UncommentedEmptyMethodBody&2\\
\cline{2-4}
 &Error Prone&BeanMembersShouldSerialize&51\\
 & &NullAssignment&11\\
 & &AvoidLiteralsInIfCondition&10\\
\cline{2-4}
 &Multithreading&DoNotUseThreads&34\\
 & &UseConcurrentHashMap&32\\
 & &AvoidSynchronizedAtMethodLevel&23\\
\cline{2-4}
 &Performance&AvoidInstantiatingObjectsInLoops&33\\
 & &RedundantFieldInitializer&23\\
 & &AddEmptyString&7\\
\hline
2018&Best Practices&JUnitAssertionsShouldIncludeMessage&39\\
 & &SystemPrintln&9\\
 & &JUnitTestContainsTooManyAsserts&5\\
\cline{2-4}
 &Code Style&MethodArgumentCouldBeFinal&27\\
 & &LocalVariableCouldBeFinal&23\\
 & &ShortVariable&10\\
\cline{2-4}
 &Design&LawOfDemeter&81\\
 & &CyclomaticComplexity&3\\
 & &ImmutableField&2\\
\cline{2-4}
 &Documentation&CommentRequired&61\\
 & &CommentSize&37\\
 & &UncommentedEmptyMethodBody&2\\
\cline{2-4}
 &Error Prone&BeanMembersShouldSerialize&64\\
 & &AvoidLiteralsInIfCondition&9\\
 & &NullAssignment&5\\
\cline{2-4}
 &Multithreading&UseConcurrentHashMap&42\\
 & &DoNotUseThreads&28\\
 & &AvoidSynchronizedAtMethodLevel&15\\
\cline{2-4}
 &Performance&ConsecutiveAppendsShouldReuse&23\\
 & &AvoidInstantiatingObjectsInLoops&19\\
 & &RedundantFieldInitializer&14\\
\hline
2019&Best Practices&JUnitAssertionsShouldIncludeMessage&42\\
 & &SystemPrintln&8\\
 & &JUnit4TestShouldUseTestAnnotation&8\\
\cline{2-4}
 &Code Style&LocalVariableCouldBeFinal&24\\
 & &MethodArgumentCouldBeFinal&21\\
 & &ShortVariable&16\\
\cline{2-4}
 &Design&LawOfDemeter&70\\
 & &CyclomaticComplexity&4\\
 & &CognitiveComplexity&3\\
\cline{2-4}
 &Documentation&CommentRequired&74\\
 & &CommentSize&25\\
 & &UncommentedEmptyMethodBody&1\\
\cline{2-4}
 &Error Prone&BeanMembersShouldSerialize&47\\
 & &AvoidLiteralsInIfCondition&12\\
 & &CloseResource&9\\
\cline{2-4}
 &Multithreading&AvoidSynchronizedAtMethodLevel&37\\
 & &UseConcurrentHashMap&30\\
 & &DoNotUseThreads&19\\
\cline{2-4}
 &Performance&AvoidInstantiatingObjectsInLoops&34\\
 & &RedundantFieldInitializer&26\\
 & &ConsecutiveAppendsShouldReuse&7\\
\hline
2020&Best Practices&JUnitAssertionsShouldIncludeMessage&24\\
 & &SystemPrintln&15\\
 & &JUnitTestsShouldIncludeAssert&11\\
\cline{2-4}
 &Code Style&MethodArgumentCouldBeFinal&27\\
 & &LocalVariableCouldBeFinal&24\\
 & &ShortVariable&10\\
\cline{2-4}
 &Design&LawOfDemeter&77\\
 & &CyclomaticComplexity&3\\
 & &AvoidThrowingRawExceptionTypes&3\\
\cline{2-4}
 &Documentation&CommentRequired&70\\
 & &CommentSize&23\\
 & &UncommentedEmptyMethodBody&7\\
\cline{2-4}
 &Error Prone&BeanMembersShouldSerialize&50\\
 & &AvoidLiteralsInIfCondition&10\\
 & &AvoidDuplicateLiterals&8\\
\cline{2-4}
 &Multithreading&UseConcurrentHashMap&37\\
 & &DoNotUseThreads&28\\
 & &AvoidUsingVolatile&16\\
\cline{2-4}
 &Performance&AvoidInstantiatingObjectsInLoops&59\\
 & &RedundantFieldInitializer&13\\
 & &ConsecutiveAppendsShouldReuse&5\\
\hline
2021&Best Practices&JUnitAssertionsShouldIncludeMessage&23\\
 & &SystemPrintln&10\\
 & &UnusedLocalVariable&9\\
\cline{2-4}
 &Code Style&MethodArgumentCouldBeFinal&30\\
 & &LocalVariableCouldBeFinal&20\\
 & &ShortVariable&9\\
\cline{2-4}
 &Design&LawOfDemeter&66\\
 & &CyclomaticComplexity&5\\
 & &CognitiveComplexity&3\\
\cline{2-4}
 &Documentation&CommentRequired&76\\
 & &CommentSize&22\\
 & &UncommentedEmptyMethodBody&1\\
\cline{2-4}
 &Error Prone&BeanMembersShouldSerialize&61\\
 & &AvoidLiteralsInIfCondition&8\\
 & &NullAssignment&7\\
\cline{2-4}
 &Multithreading&AvoidSynchronizedAtMethodLevel&42\\
 & &UseConcurrentHashMap&26\\
 & &DoNotUseThreads&18\\
\cline{2-4}
 &Performance&RedundantFieldInitializer&25\\
 & &AvoidInstantiatingObjectsInLoops&22\\
 & &ConsecutiveAppendsShouldReuse&15\\

\end{tabular}
\label{javacodesmellcount}
\end{center}
\end{table*}

==> deprecated/IEEE-old/sections_abandoned/RQ3.tex <==
\subsection{RQ3 Maintenance}
The adoption of a paper is an endorsement of the research work but isn't a signal of the end of it. After the adoption, active maintenance of the artifact and prompt response to users' questions are also important to ensure reproducibility. Thus, RQ3 studies the maintenance situation in the past five years from the perspective of maintenance time and dead URLs.

\subsubsection{RQ3.1 Maintenance Time}
For users, the last update time of artefact helps them judge whether the artefact is useful. Recently maintained artefacts are more popular with users. RQ3.1 studies the maintenance time of artefacts.

We checked all artefacts that were able to keep track of when they were updated. Due to the different deadlines for different conferences of different years, it is necessary to list the situation of each conference in the past five years separately. Table \ref{Last update time} shows the updates of the artefacts included in the conference of the same year.

\begin{table*}[htbp]
\caption{\upshape{How many artifacts are last-updated during this quarter}}
\begin{center}
\begin{tabular}{|p{20mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|p{1.5mm}|}
\hline
conference&\multicolumn{4}{c}{ASE}&&\multicolumn {4} {c} {FSE}&&\multicolumn {4} {c} {ICSE}&&\multicolumn {4} {c} {ISSTA}&\\
\hline
\diagbox{\makecell[l]{last\\ update\\time}}{\makecell[l]{held\\year}}&17&18&19&20&21&17&18&19&20&21&17&18&19&20&21&17&18&19&20&21\\
\hline
2022.7-2022.8&1&3&0&2&0&1&2&2&5&0&3&2&0&0&1&0&2&0&2&1\\\hline
2022.4-2022.6&0&1&1&3&10&1&0&0&3&6&0&2&3&1&5&0&2&2&1&3\\\hline
2022.1-2022.3&2&1&1&1&4&1&0&2&2&8&0&0&2&0&6&0&0&0&0&1\\\hline
2021.10-2021.12&0&0&1&3&\cellcolor{yellow}8*&1&1&2&0&5&1&1&3&1&5&0&0&0&1&7\\\hline
2021.7-2021.9&0&1&2&1&21&0&1&2&1&\cellcolor{yellow}29*&0&0&0&2&3&1&0&0&2&\cellcolor{yellow}5*\\\hline
2021.4-2021.6&0&1&0&3&4&0&0&0&5&14&0&0&1&7&\cellcolor{yellow}6*&0&0&2&1&14\\\hline
2021.1-2022.3&1&0&0&4&0&1&0&1&3&9&0&0&5&1&36&0&0&0&2&4\\\hline
2020.10-2020.12&1&1&1&4&0&0&0&2&\cellcolor{yellow}5*&0&0&1&1&3&2&0&1&0&4&0\\\hline
2020.7-2020.9&1&2&3&\cellcolor{yellow}19*&0&1&1&2&13&0&0&2&2&0&6&0&1&0&\cellcolor{yellow}4*&0\\\hline
2020.4-2020.6&0&0&2&5&0&0&1&1&15&0&0&0&1&\cellcolor{yellow}5*&0&1&1&0&6&0\\\hline
2020.1-2020.3&2&2&3&5&0&0&1&2&2&0&0&3&0&13&0&1&1&1&0&0\\\hline
2019.10-2019.12&0&0&\cellcolor{yellow}4*&0&0&2&1&3&0&0&0&2&1&0&0&0&0&1&0&0\\\hline
2019.7-2019.9&2&3&8&0&0&0&1&\cellcolor{yellow}8*&0&0&0&3&3&1&0&0&2&\cellcolor{yellow}3*&1&0\\\hline
2019.4-2019.6&2&3&4&0&0&0&2&3&1&0&0&1&\cellcolor{yellow}1*&0&0&0&0&3&0&0\\\hline
2019.1-2019.3&2&2&1&0&0&0&1&3&0&0&0&3&15&1&0&0&1&0&0&0\\\hline
2018.10-2018.12&1&1&0&0&0&0&\cellcolor{yellow}6*&0&0&0&0&0&1&0&0&1&1&0&0&0\\\hline
2018.7-2018.9&0&\cellcolor{yellow}6*&0&0&0&2&11&0&0&0&0&2&1&0&0&0&\cellcolor{yellow}1*&0&0&0\\\hline
2018.4-2018.6&0&2&0&0&0&1&4&0&0&0&0&\cellcolor{yellow}3*&0&0&0&0&1&0&0&0\\\hline
2018.1-2018.3&1&0&0&0&0&4&3&0&0&0&1&12&0&0&0&2&1&0&0&0\\\hline
2017.10-2017.12&\cellcolor{yellow}4*&0&0&0&0&0&0&0&0&0&1&0&0&0&0&0&0&0&0&0\\\hline
2017.7-2017.9&4&0&0&0&0&\cellcolor{yellow}1*&0&0&0&0&1&3&0&0&0&\cellcolor{yellow}2*&0&0&0&0\\\hline
2017.4-2017.6&3&0&0&0&0&4&0&0&0&0&\cellcolor{yellow}2*&0&0&0&0&0&1&0&0&0\\\hline
2017.1-2017.3&0&0&0&0&0&1&0&0&0&0&3&0&0&0&0&0&0&0&0&0\\\hline
past-2016.12&1&0&0&0&0&0&0&0&0&0&3&1&0&0&0&0&0&0&0&0\\\hline
\end{tabular}

The yellow cell with a ``*'' indicates the time of the conference.
\end{center}
\label{Last update time}
\end{table*}

According to the Table \ref{Last update time}, the artefacts whose last update time are within 4 months before conferences accounted for \draft{50\%}. \draft{number\%} of artefacts were still maintained after the meeting and the maintenance time for \draft{90\%} of them are within one year after the conference. It illustrates that most artefacts are accustomed to intensively updating within four months before the conferences, while a small number of artefacts will continue to be actively maintained in one year after the conferences. Noted that there are fewer than \draft{35} accepted papers in ISSTA, so relatively few ISSTA artefacts can be tracked to maintain information.

\textbf{Finding 10}:
The last update time of 60\% of artefacts is concentrated in 4 months before the conferences and within one year after the conferences.

\subsubsection{RQ3.2 Dead URLs}
Although some artefacts have not been updated for a long time, their URLs are still alive. However, some URLs of artefacts have been dead over time, resulting in missing artefacts. Therefore, RQ3.2 answers the question of how many URLs of artefacts have been dead until now.

\quest{the content of RQ3.2}

As Figure \ref{deadurls} shows, the number of dead URLs has increased slowly over time. Further more, \draft{number\%} of dead URLs, which are URLs of homepages created by the authors, are caused by the homepage being stopped maintenance. \draft{number\%} of the dead links are shared links of cloud disks, and the links are invalid due to the expiration of the shared links.\draft{need to modify}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/3-2/Figure_10.png}
\end{center}
\caption{The number of dead URLs from 2017 to 2021.\jie{Revise, detailed comments in wechat group}}
\label{deadurls}
\end{figure}

Although invalid URLs are only a small fraction of all artefacts, which is 10\%. However, the URL of the artefact cannot be updated in a paper after the URL failed, which is not conducive to the continued research. Therefore, keeping the URLs of artefacts alive is also an important aspect of artefacts maintenance.

\textbf{Finding 11}:
Over 7.2\% of URLs in artefacts of each year have been invalid until now. And 19.4\% of URLs of artefacts of 2017 have been invalid, which is a ratio that worth noting.

\begin{tcolorbox}
\textbf{\underline{Answer to RQ3:}} 
\draft{50\%} of artefacts were last updated within 4 months before the conferences from 2017 to 2021. The proportion of artefacts that are still maintained actively after the conferences has increased year by year, reaching \draft{30\%} in 2021. However, over \draft{5\%} of URLs of artefacts have failed over time, with \draft{20\%} of dead URLs in artefacts of 2017.

\end{tcolorbox}

==> deprecated/IEEE-old/sections_abandoned/RQ4.tex <==
\subsection{RQ4 Top-Starred Artefacts}

The number of stars is an important indicator of the popularity of a project in the open source community. For the replication repository of the paper artifact, the higher the number of stars, the more popular the repository is, and the higher the project quality and code quality may be. Therefore, RQ4 explores the characteristics of top-starred repositories to guide the development of future replication repositories.

\subsubsection{RQ4.1 Star Situation}

RQ4.1 first studies the star situation of artefacts each year, by making statistics on the number of stars of artefacts from 2017 to 2021 and drawing violin diagrams based on the statistical results. As shown in the right of Figure \ref{starsviolin}, the highest star numbers of artefacts from 2017 to 2021 are \draft{number}, \draft{number} 3200, 964 and 139, respectively. It illustrates the artefacts of earlier time may have the higher number of stars. But for \draft{number\%} artefacts, the number of stars is concentrated in the range of 0 to 10. In fact, there are only two artefacts with more than 300 stars, one of which is the artefact of the paper \cite{} published on FSE in 2019. The artefact had surpassed 2500 stars as its corresponding paper published and had more than 3200 stars at the time of statistics. The other artefact, corresponding to the paper \cite{} published on FSE in 2020, has 964 stars at the time of statistics.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/4/tmp4-1.png}
\end{center}
\caption{The violin diagram of stars of github repositories from 2017 to 2021.}
\label{starsviolin}
\end{figure}

What's more, in order to observe the overall distribution of star numbers, we need to remove outliers with too many stars. After removing the artefacts with the most stars from 2017 to 2021, the maximum number of stars in the remaining artefacts does not exceed \draft{274}. The violin diagram is shown in the left of Figure \ref{starsviolin}. It can be seen that both the mean and the median number of stars of artefacts have decreased year by year, probably due to the earlier artefacts have been open source for longer time. In addition, \draft{60\%} of artifacts have less than 10 stars, and \draft{50\%} of artefacts have less than 1 star.

\textbf{Finding 12}: Only \draft{number} artefacts have a high star count of more than 300, while the artefacts whose star number can be counted with two hands account for over \draft{80\%}.

\subsubsection{RQ4.2 Characteristics}

RQ4,2 focuses on the characteristics of the top-starred artefacts. The top 5 artefacts of each year sorted by number of stars from 2017 to 2021 are labelled as top-starred artefacts. Three aspects of characteristics of the top-starred artefacts, including content, code quality and maintenance, are analysed.

First, from the content point of view, among the 15 top-starred artefacts, 14 artefacts contain code and implement tools, and 1 artefacts only contains data. Second, \draft{number} of the 14 repositories that contain code, 4 contain data and 6 contain tests for code. Third, each of the 15 top-starred artefacts provides detailed documents, including project introduction, installation instructions, usage methods, and examples. Fourth, 13 of the 15 artefacts have licenses. Fifth, from the perspective of code language, 4 artefacts use more than 10\% python language, 4 artefacts use java language, 4 artefacts use C/C++ language. And 7 artefacts use only one language (2 use Python, 3 use Java, 1 use F\# and 1 use Haskell).

From the perspective of code smell, first, the average number of messages in top-starred Python artefacts, \draft{number\%}, is much lower than the overall average number, \draft{number\%}. It shows that top-starred artefacts have higher code quality. The most common problems of top-starred Python artefacts are three Convention Messages including invalid-name, line-too-long and missing-function-docstring. Second, in the 4 top-starred java artefacts, the number of code smell problems in Java artefacts with relatively higher star numbers (3200, 964 and 139) is lower than \draft{number}, which is significantly lower than the average number of corresponding year\footnote{The average number of code smell problems in Java artefacts is \draft{number}, \draft{number}, \draft{number}, \draft{number} and \draft{number} from 2017 to 2021 respectively.}. The code smell problems in top-starred artefacts are simmilar to most artefacts, which are concentrated on Code Style problems including LocalVariableCouldBeFinal and MethodArgumentCouldBeFinal.

In terms of maintenance, 3 of 5 top-starred artefacts in 2019 are still maintained after June 2021. There are 4 top-starred artefacts in 2020 still under maintenance in 2022. 4 of the 5 top-starred artefacts in 2021 are still maintained after November 2021.

\draft{Need Table here?}

\textbf{Finding 13}: \draft{70\%} of top-starred artefacts contain both code and data and implement popular tools. All of the 25 top-starred artefacts contain documentation, and \draft{15} contain tests written for code. There are \draft{20} artefacts that are still updated or maintained one year after the conferences. \draft{10} Python artefacts and \draft{number} Java artefacts have high code quality while their common code smell problems are similar to most artefacts.

\begin{tcolorbox}
\textbf{\underline{SUMMARY 4:}} 
\draft{90\%} of artefacts have no more than 50 stars, while 25 top-starred artefacts have no less than 80 stars and the highest star count of them exceeds 3,200. Of the top-starred artefacts, more than \draft{70\%} implement tools and contain code with good code smell, data, documentation and tests for code with high content integrity and high usability. \draft{80\%} of top-starred artefacts are still being maintained until 2022, with a good maintenance situation.
\end{tcolorbox}

==> deprecated/IEEE-old/sections_abandoned/background.tex <==

Generally speaking\draft{actually in my opinion...}, the life cycle of an artefact includes four stages: preparation, quality evaluation, maintenance, and possible popularity. At each stage, researchers face different choices and encounter various problems. Therefore, our research questions(\textbf{RQ}) cover the four stages of artefact. In addition, we divide each stage into several sub-research questions to describe the current situation of artefact in detail.
\jie{todo for Jie: make RQs a big table}

\noindent\textbf{\underline{RQ1 Preparation}: What are the common practices for software engineering researchers to prepare their artefacts? }
How to prepare artefact is an important question that artefact builders need to answer first. In preparation stage, researchers need to consider whether to build an artefact, where to open source it, how to give the artefact's address, what should be included in the artefact, and what code language to use. Therefore, with these five questions, we describe the general situation and summarize the general mode and common problems encountered in the preparation process of artefact.\\
\noindent \emph{\underline{RQ1.1 \jie{make this a seperate RQ}Ratio of Papers with Artefact}: How does the ratio of papers with artefact change in the past 3 years? }
From 2017 to 2021, chairmen have spent much effort calling on researchers to build their artefact of paper. So RQ1.1 wants to figure out how these efforts paid off.\\
\noindent \emph{\underline{RQ1.2 Storage Website}: What websites are used to upload the artefacts? }
Using a popular open source platform to manage artefacts including code and data means that it can be more easily used by more users, and it would be convenient to compare different artefacts. Therefore, RQ1.2 explores what platform researchers like to use to manage their open source artefacts.\\
\noindent \emph{\underline{RQ1.3 URL Position}: In which position in a paper do researchers provide the artefact URL? }
After establishing the artefact, researchers need to consider how to provide the URL of artefact. This question is important because readers can easily ignore the URLs of artefacts that given in inconspicuous positions of paper. At the same time, finding these inconspicuous artefacts costs readers a lot of extra time. RQ1.3 discusses where researchers provide artifact URLs in their papers.\\
\noindent \emph{\underline{RQ1.4 Content}: What do the artefacts contain? }
To ensure reproducibility, all data, code and results should be included in the artefact. However, due to space constraints, legibility and other reasons, not all content will be open sourced in artefact. RQ1.4 explores the content of the artefact and analyze whether the content can guarantee the paper's reproducibility.\\
\noindent \emph{\underline{RQ1.5 Programming Language}: What programming languages are used in artefacts? }
Programming language is a vital feature of code. RQ1.5 figures out which programming language researchers like to use in artefacts.\\
\noindent\textbf{\underline{RQ2 Quality}: How good are the practices of preparing the artefacts? }
The quality of artefacts is the core concern of reproducibility. This paper analyzes the quality of artefacts from two aspects: content integrity and code quality. In terms of content integrity, we pay attention to whether the artefact has readme documents, which affects the usage and reproduction, and test code, which is related to the possibility of potential bugs in the code. In terms of code quality, we count the code smells of artefacts of two common languages, python and java, to explore the code quality.\\
\noindent \emph{\underline{RQ2.1 Documentation}: Do the repositories have detailed readme documents? }
Detailed readme documents introduce the content, installation, usage of the code and data of artefacts. The reproducibility of artefacts cannot be ensured easily without readme documents. Hence, RQ2.1 focuses on the documentation  situation of artefacts\\
\noindent \emph{\underline{RQ2.2 Tests}: Do researchers write tests for the code in the artefacts? }
Testing code is essential in the field of software engineering. Untested code can often have many potential bugs. Therefore, RQ2.2 explores whether the code in the artefacts has been tested by counting whether test code is stored in artefacts.\\
%\draft{remove RQ2.3: Do the repositories provide docker images?}\\
\noindent \emph{\underline{RQ2.3 Code Smell}: What are the code smells in the artefacts? }
Code smell is a primary indicator of code quality. Good code smell means high code quality. Therefore, RQ2.3 uses code smell detection tools to detect different aspects of code smell to explore the code quality of artefacts.\\
\noindent\textbf{\underline{RQ3 Maintenance}: How well do researchers maintain their artefacts? }
The maintenance situation of artefacts is a quality indicator that can not be ignored. As a repository is open sourced, researchers may need to update their data, code and documents according to uses' responses. Therefore, RQ3 explores the change of maintenance situation in past five years from the perspective of maintenance time.\\
\noindent \emph{\underline{RQ3.1 Maintenance Time}: How long do researchers actively maintain their artefacts?}\\
\noindent \emph{\underline{RQ3.2 Changes of Maintenance Situation}: How does the maintenance situation change in the past five years?}\\
\noindent\textbf{\underline{RQ4 Top-Starred Artefacts}: What are the characteristics of top-starred replication repositories?} Repositories with high stars tend to mean high popularity. Therefore, RQ4 studies the popularity of artefacts by counting the number of stars. What's more, RQ4 explores the characteristics of top-starred artefacts, which can serve as a reference in the future construction of artefacts.\\
\noindent \emph{\underline{RQ4.1 Star Situation}: How is the star situation of artefacts?}\\
\noindent \emph{\underline{RQ4.2 Characteristics}: What are the common characteristics of top-starred artefacts?}\\

==> deprecated/IEEE-old/sections_abandoned/conclusion.tex <==

% conclusion

\textbf{interesting findings}

\textbf{echo contribution}

==> deprecated/IEEE-old/sections_abandoned/discussion.tex <==

\section{Discussion}

\draft{feel that these two subsection cannot be placed in one section and need to be adjusted, so there are not summary.}

\subsection{Life Cycle Pattern and Future Consideration}
This paper divide the life cycle of artefacts into four parts to analyse the general situation of building an artefact in the field of software engineering. As the quantity and quality of artefacts have gradually increased from 2017 to 2021, there are still some hard bones in the life cycle of artefacts that may trouble researchers. We list these problems below to point out a reference direction for further optimizing the construction environment of artefact.

\emph{What kind of content to upload to artefact?}
For copyright or confidentiality reasons, \draft{number\%} artefacts does not open source its code or data, which is a great damage to the reproducibility of artefacts. Therefore, during the construction of open source artefacts, necessary codes and data should be uploaded as much as possible to restore the experimental process to ensure reproducibility.
However, How can we ensure the reproducibility of artefacts when the data is confidential? It's still a difficult problem that needs researchers' further consideration.

\emph{Where to store data that take up a large amount of storage?}
As more and more research is driven by data, the data of many artefacts needs large storage space. However, the current commonly used storage website GitHub can not meet the needs of big data. Therefore, where to store the data is a problem that many researchers may have encountered. There are mainly three ways to solve this problem currently. One is to share data links using cloud disk, although the shared URL is easy to fail. The second is to use personal websites for sharing, which requires researchers to pay effort and money to maintain personal servers. The third is to use Zenodo for sharing. Zenodo is a well-known data sharing platform and the data can be saved for life, with the space limit up to 50GB, which is suitable for sharing the data and code of artefacts. As the current big data storage websites are messy, it is difficult for users to access data and compare similar data of different artefacts conveniently. Therefore, we recommend using Zenodo to store large amounts of data 
of artefacts.

\emph{How to build a long term link for artefacts?}
URL cannot be updated in published paper. So we recommend that researchers use storage sites that support persistent repository URLs, such as Github and Zenodo. When it's needed to use other storage websites, it's must to consider whether the URL of artefacts will still work over time?

\emph{Is test necessary for artefacts?}
Tests for code of artefacts are easily overlooked according to our study. However, sufficient tests can ensure that the tools can be used more smoothly, the code for data analysis works correctly, and the results are reliability in artefacts. So we recommend writing enough tests for the code in artefacts.

\emph{The star of artefacts is 0, do I still need to maintain it?}
Maintenance situation is not optimistic, as many artefacts stopped maintenance as the conference finished. Artefacts that lack maintenance may reduce the reliable and not be accepted by users. In this case, users may choose to implement the code of artefacts themselves or use other actively maintained recurring open source repositories. Good maintenance helps the project stay alive. Regular feedback, updates, and answering questions will not only help latecomers make better use of these projects, but also help them get more stars. We recommend that researchers maintain artefacts regularly.

\emph{How to improve the code quality of artefacts?}
There are large amounts of code smell problems in most artefacts, which illustrates that Code quality is an overlooked problem. To improve the code quality of artefacts, we recommend using static code analysis tools when developing artefacts.

\subsection{How to build a top-starred artefacts?}

\draft{give advice on how to build a good artefact. Detailed guidance.}

Guidance for each of the three stages.

\emph{Preparation}
1 upload content as full as possible, and organize in clear form.
2 make data and code easy to use. data need to download, check, parse, use easily. code need to install, use easily.
3 choose well known and popular website
4 show URL in an easy-to-find position in paper. 
5 Use programming language commonly used by peer researchers

\emph{Quality Improvement}
1. write document in details, including introduction, installation and use instruction, description of files in artefacts.
2. write test for code.
3. use static code analysis tools to help when coding.

\emph{Maintenance}
1. Keep the origin link alive
2. Respond to users' questions and updates in time

\emph{Popularity}
1. Publicity and active maintenance.

\subsection{What kind of artefacts are good?}

Artifacts are designed to ensure reproducibility, so artifacts with good reproducibility are good.

1 correctness: content, storage website, programming languages. test

2 easy-to-understand: documentation, code smell

3 easy-to-use: documentation, good-maintenance, (docker or pip )package

\subsection{Bad artefacts and its proportions}
We can use some metrics to evaluate the problem artefacts, including URL/website condition, content, maintenance, popularity. 

First, from the perspective of URL/website condition, the artefacts with below situation are poor.

1. Artefacts that hide its URL in paper, with propersition of \draft{number\%}

2. Artefacts with failed URL

Second, from the perspective of content, these artefacts are not good enough:

3. Artefacts that only have brief document.

4. Artefacts with no document.

5. Artefacts with code but no tests.

6. Artefacts with bad code smell.

Last but not least, artfacts with no maintenance and no star have poor availability
 from the perspective of maintenance and popularity.




==> deprecated/IEEE-old/sections_abandoned/introduction.tex <==
\jie{a very related paper we previously missed~\cite{ChristopherTimperley2021}}

Reproducibility is the basis of a research work. A paper's results cannot be reproduced means that the research has not see through the essence and The knowledge it presents is untenable. \jie{also mention the attention from other domain, such as the discussions on reproducibility crisis in ~\cite{baker20161}}In recent years, many chairmen in the field of software engineering have called for research artefacts to enhance the reproducibility of papers\cite{hermannCommunityExpectationsArtifacts2020}. At the same time, the reproducibility of papers has received great attention from researchers\cite{liuReproducibilityReplicabilityDeep2022}\cite{ mendez2019artefacts}\cite{dacremaAreWeReally2019}. As shown in the Figure \ref{ratioofpaper}, with the joint efforts of researchers, the number of paper with artefact in top conference papers in the field of software engineering has increased rapidly in the past five years . The proportion of paper with replication packages in all papers has increased from 59.1\% in 2017 to 79.5\% in 2020 and 68.9\% in 2021, which means most of papers provide a replication package for other researchers to verify and apply. The concept of artifact, which is described as \draft{need the definition of artifact}, was proposed by Méndez et al.\cite{mendez2019artefacts} in 2019.

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=1\textwidth]{pics/1-1/Figure_1-1.png}
\end{center}
\caption{\jie{to discuss: reorganise the graph}The number of papers with and without artefacts in each conference from 2017 to 2021.
%\draft{font size too small and also need to use textures to distinguish different data.}
}
\label{ratioofpaper}
\end{figure*}

\jie{say something like: there are certainly many interesting points to dig deep into in this direction. It is impossible for us to cover them all in one single paper. This paper does not aim to provide a comprehensive and deep analysis of each aspect. Instead, we aim to provide an overview of the current status of artefacts in SE. We hope that our work can arouse more interest from the community to work on this direction and provide more systematic and deep studies.}


In addition, the quality of artefacts also affects the reproducibility of papers. On the one hand, although most software engineering papers provide research artefacts, it is often difficult for users to distinguish the quality of these artefacts. In particular, the artefacts corresponding to papers on software and system usually contain a large amount of code and data. These artefacts are expected to have good code quality, can be deployed and run correctly, have detailed documentations, and be 
fully tested. Otherwise users may encounter a series of problem when using these artefacts for verification and application. On the other hand, there is not much guidance on how to improve the quality of the artefacts. Therefore, the artefacts tend to have a strong personal style of authors, which is also not conducive to users' learning and reuse.

Although the quality of artefacts play an important role, to the best of our knowledge, in the software engineering community, there is currently no empirical research on the characteristics of research artefacts, including quality. In fact, empirical analysis is the basis of software engineering research \draft{need citation here}. Through empirical research on the characteristics of software engineering artefacts, we could have a better understanding of the current artefact situation and guide the artefact community to develop in a higher quality.

To bridge this knowledge gap, we make a empirical study on the situation of artefacts in software engineering area in past five years. From the perspective of the life cycle of artefact, our study investigates four aspects of artefact, including the \textit{Preparation} (RQ1), \textit{Quality} (RQ2), \textit{Maintenance} (RQ3) of artefacts and the \textit{Characteristics of Top-Starred}(RQ4) artefacts. 
First, to reveal the preparation process of artefacts, we conduct a statistical analysis of the artefacts from the perspectives of content, open source location, and code language. Second, in order to measure the general quality of artefacts, we focus on whether there is documentation in artefacts, whether there is tests written for the code and the code smell of artefacts containing code. Code smell in artefacts are measured and counted by dedicated tools. Third, by marking the last update time of artefacts, we statistically analyze the active maintenance time of artefacts, and the changes in the maintenance situation in the past five years. Fourth, we explore characteristics of top-starred artefacts to provide a reference for the future direction for improving the quality of artefact. To our best knowledge, these four aspects comprehensively reflect the current situation of artefacts in software engineering community. \draft{May be we need citation here?}

In order to answer these questions, this research first collects a total of 1552 papers from main track of the four conferences of \textit{International Conference on Software Engineering} (ICSE), \textit{ACM SIGSOFT Symposium on the Foundation of Software Engineering/ European Software Engineering Conference} (FSE), \textit{International Conference on Automated Software Engineering} (ASE), and \textit{International Symposium on Software Testing and Analysis} (ISSTA) from 2017 to 2021. Figure \ref{ratioofpaper} shows the number of papers we collected in this four conferences from 2017 to 2021, respectively. These four conferences are the top conferences in the field of software engineering, which can reflect the ecology of the current highest level in the field of software engineering. Then, among these papers, we find the open source addresses of a total of 1552 artefacts by combining keyword search and manual checking. After that, we manually mark the storage platform, contents, maintenance interval, code language and the number of stars of artefacts if they have. Finally, by analyzing these features, the above four research questions (RQs) can be answered.

\draft{Findings in bold are potentially interesting (for drafts only)}

After analyzing the data we collect, this paper has the following findings. First, \draft{can remove?}data and code are the most common content in artefacts, accounting for 48.3\% and 85.2\% of artefacts respectively. \textbf{33.5\% of artefacts contain both data and code while \draft{number\%} of artefacts only have a brief introduction}. \textbf{Besides, \draft{number} researchers prefer to put their code on github, while data may be placed in various places}. Second, \textbf{researchers pay much attention to documentation but not enough for writing tests for the code}, as 96.5\% of artefacts have documents while 23.7\% of artefacts have tests for their code. What's more, no matter what code language is used, \textbf{conventional code style rules and documentation are two most overlooked code smells}. Third, \textbf{55.8\% of artefacts stop maintenance after papers' publication. 16.4\% of artefacts are still maintained one year after papers' publication}, and \draft{need ensure} this proportion is increasing year by year. Fourth, \textbf{\draft{number\%} artefacts have less than 10 stars}. More than \draft{90\%} of top-starred artefacts have license, detailed documents and over one year of maintenance after papers' publication. \draft{99\%} of top-starred artefacts provide tools and \draft{80\%} of them have \draft{70\%} less code smell issues than average.
%after 427/967 continue maintenance 44.2%
%after 1 year 159/967 16.4%

In summary, the main contributions of this paper are listed as follows: \draft{the red lines in this place must be echoed later}
\begin{itemize}
    \item We are the first to conduct an empirical analysis of the content of the papers' artefacts. Our empirical analysis reflects the overall situation of the whole life cycle of artefact from preparation, quality, maintenance, to popularity. \draft{This empirical study provides evidence for researchers to further study the artefacts of papers.}
    \item From the perspective of life cycle, we do a comprehensive analysis of the situation of artefact. And each life stage is described by several sub-research questions in detail. Further, based these analysis, \draft{in \textit{Discussion} section,}we put forward the problems that may be encountered in current artefact life cycle and \draft{point out a reference direction for further optimizing the construction environment of artefact.}
    \item We analyze the characteristics of top-starred artefacts and \draft{give advice on how to build a good artefact}. These characteristics include three aspects of content preparation, content quality, and maintenance time. For future artefact builders, these characteristics provide detailed and specific guidance to improve the quality of artefacts.
\end{itemize}

This paper is organized as follows. Section 1 briefly introduces the research motivation, research questions, research methods, conclusions and possible implications of this paper. Section 2 introduces the research background and research questions of this paper in detail. Section 3 introduces the research method of this paper in detail, as well as the processing details in the process of data collection, data processing and data analysis. Section 4 introduces the research results of this paper, and gives the answers to the research questions raised in the second chapter through the analysis of the data. [Section 5]. Section 6 introduces the related work of this paper, including the related work of Research Artifacts and software empirical research. Section 7 summarizes the main conclusions of this paper and the possible implications of these conclusions.



==> deprecated/IEEE-old/sections_abandoned/methodology.tex <==
To answer all these research questions, we downloaded 1,552 papers and screened \draft{number} papers with artefacts for study. Then, we manually labelled 11 characteristics for further analysis. In particular, we detected the code smells of Python artefacts and Java artefacts by code smell detection tools to quantify the code quality of artefacts.

\subsection{Collection of Papers/artifacts}
We collect SE papers that provide artifacts as the research subject of our study. To this end, we downloaded a total of 1,552 papers from the research track of four top-tier conferences in the SE community, including ICSE, FSE, ASE, and ISSTA, from 2017 to 2021. 

We searched for the URL of artefact in the papers by keyword searching combined with manually searching.
Specifically, we define multiple search keywords to help us quickly locate the URL, including ``http'', ``replication'', ``github'', ``code'', ``data'', ``available'' and ``share''. In this way, we have collected \czp{xxx} papers that provide artifacts. For the remaining papers, we manually check them to avoid the omissions and thus obtain \czp{xxx} additional papers with artifacts.
% because the URL of artefact may appear in various forms \czp{what does ``forms'' refer to?} in different positions of paper, we search the URL of artefact by multiple keywords, including ``http'', ``replication'', ``github'', ``code'', ``data'', ``available'', ``share'' and ``republication''.
% On the other hand, to avoid omissions as much as possible, we search for the URL of artefacts by manually reading the paper when the URL cannot be found by keywords searching. While reading, We focus on the abstract, the introduction and the end of paper, three places where URLs tend to appear.

We manually examine each of the \czp{xxx} papers collected to filter those whose artifact URL does not work. As a result, we have a total of \draft{number} papers for our study.
% we manually checked whether the search results are the URL of artefacts corresponding to papers and whether the URLs still work. Then, we build our data set consisting of 1055 papers with artefact.
Fig. \ref{ratioofpaper} shows the number of papers with artefacts in each conference from 2017 to 2021.

\subsection{Analysis of Artifacts}
We then analyze the collected artifacts to answer the research questions.

For each artefact, we extract 11 characteristics, including publication year, conference, paper title, URL position in paper, description, archive site, programming language, maintenance, stars, document quality, test quality, and code smell.
\czp{why do you use ``has-document''? I think it is not a binary characteristic, i.e., with or without document.} \draft{because we only label whether the artifact have document or not qwq} Next, we describe the extraction of each characteristic briefly.
% and three content-aspect characteristics (i.e., has-documents, has-tests and code smell.

For the first 5 characteristics, in the process of searching for the URL of the artefact in the paper, we mark the publication year, conference, paper title, the URL position in paper and the description of the artefacts in the paper. For the URL position in the paper, we roughly divide it into five categories: Abstract, Introduction, Body, End, and Reference. If the URL appears multiple times, only the first occurrence will be recorded. In addition, when the paper gives the URL of the artefacts, a short description of artefacts is often attached, and we record this description as the artefact's description.

We entered the artefacts in turn to manually label the last 6 characteristics. The storage websites of artefacts are easily tagged after entering the artefacts' repositories. Then, because most storage websites will display the proportion of code languages and star number of artefacts, we mark the proportion of code languages and star number of artefacts according to the display of the storage websites. We ignore these two characteristics if the storage website does not display the information. Totally, 673 artefacts' code language and star information are labelled. Java and python are the top 2 most used programming languages in artefacts, occupying 29.8\% and 51.1\% respectively.
For the maintenance time, we take the author's latest response time as the last maintenance time, which includes the latest file update time, the latest issue response time and the latest request processing time. 
In terms of content-aspect characteristics, we observe all files in artefacts, and manually find and mark the documentations and files of tests written for code. Besides, code smell detection tools are used to obtain the code smell of artefacts, which will be introduced in detail later.

\subsection{Code Smell Detection}

\subsubsection{Data Preprocess}

Only code smells of artefacts with Python or Java usage over 10\% were detected. There are two reasons. On the one hand, the proportion of python and java is 29.8\% and 51.1\% respectively, occupying most of the code of artefacts. And the proportion of other languages, including C/C++, is only 20.1\%. Hence the code smell of these two languages is enough to reflect the overall code smell situation of artefacts. On the other hand, only python and java are used by more than \draft{number} artefacts with usage proportion over 10\% every year. Thus, it's convenient to analyze the changes of code smell situation in past five years by detecting the code smell of python and java. Therefore, we only detect the code smell of artefacts using these two languages, python and java. Furthermore, to improve detection quality, we only detect artefacts with Python or Java usage over 10\%. Finally, \draft{number} artefacts with Python usage over 10\% and \draft{number} artefacts with Java usage over 10\% are obtained.

Further, our goal is to detect code smells of code used in the research process written by the researchers themselves. However, in artefacts, there are still some code files that don't meet this requirements, including the code files used as analysis data, the data files that stored in code formats, the code files of the external tools used in artefacts, and the code files of environment. Therefore, we check the code files in the artefacts one by one and exclude the code files of these cases. 

In short, the artefacts whose code smells are detected must meet the following two requirements. First, the usage ratio of Python or Java exceeds 10\%. Second, the code of Python or Java in artefacts must be written by the researchers of artefacts and used in the research process. Finally, we get \draft{number} Python artefacts and \draft{number} Java artefacts, all of which meets all the above requirements.

\subsubsection{Code Smell Detection Tools}
There are many commonly used code smell detection tools for Python and Java. Considering both popularity and convenience, Pylint and PMD are chosen to detect the code smell of Python artifacts and Java artefacts respectively.

Pylint, whose github repository has 4,144 stars, is a tool dedicated to Python code quality detection and is widely used in Python code inspection. Pylint classifies code quality issues of Python into 6 categories: \textit{Fatal Message}, \textit{Error Message}, \textit{Warning Message}, \textit{Convention Message}, \textit{Refactor Message}, and \textit{Information Message}. The Fatal Message indicates that some errors occurred during detection that prevent Pylint from continuing to run, such as an exception occurred. The Error Message indicates that an error was found while detecting, such as Pylint has been unable to import a module. The Warning Message include unused-variable, bad-indentation and other warning messages. The Convention Message indicates that the code style does not conform to the convention, including invalid-name, etc. The Refactor Messages include duplicate-code, too-many-arguments, etc. And the Information Message are relatively rare, mainly including c-extension-no-member and so on. These messages can reflect the code quality of various aspects of Python code.

PMD is a commonly used tool that can support cross-language static code detection in multiple languages, including java, JavaScript, etc. And PMD is often used for static detection of code smell of java, and its github repository has 3.9k stars. The rules of java code in PMD are divided into eight aspects: \textit{Best Practices}, \textit{Code Style}, \textit{Design}, \textit{Documentation}, \textit{Error Prone}, \textit{Multithreading}, \textit{Performance} and \textit{Security}. Among them, Best Practice provides rules which enforce generally accepted best practices, including JUnitAssertionsShouldIncludeMessage and so on. Code Smell refers to rules which enforce a specific coding style, including LocalVariableCouldBeFinal and so on. Design rules help users discover design issues, including LawOfDemeter, etc. Documentation rules are related to code documentation. Error Prone includes rules to detect constructs that are either broken, extremely confusing or prone to runtime errors. Multithreading provides rules that flag issues when dealing with multiple threads of execution. Performance is responsible for flag suboptimal code. And Security includes rules that flag potential security flaws.

\draft{Actually, PMD also provide the priority of each code smell, but we didn't analysis this aspect. We can add it if necessary.}

==> deprecated/IEEE-old/sections_abandoned/related.tex <==
This section first introduces previous work about research artefact. Then, we demonstrates the empirical study of code repository, mostly Github. Finally, we show the differences between our study and mentioned work. And we illustrate the highlights of our work.

\draft{emphasize that many researchers pay attention to this area.}

\jie{add related work~\cite{damasceno2021towards}}
\subsection{Research Artefact}
A lot of early work, such as \cite{biggs2002role},\cite{makela2007knowing},\cite{lowry2017security},\cite{gravelle1998much},\cite{currie2009contextualising},\cite{riemer2014rethinking},etc , mentioned artefacts, but for a long time there was no clear definition of what an artefact was. M{\'e}ndez Fern{\'a}ndez and co-authors' work\cite{mendez2019artefacts} in 2018, focused on what artefacts are, provided a positioning and critical reflection upon the notion of artefacts in software engineering at different levels of perception and how these relate to each other. They further contributed a metamodel that provides a description of an artefact that is independent from any underlying process model. The metamodel defines artefacts at three levels: Semantic Content, Syntactic Structure and Physical Representation. Abstraction and refinement relations between these levels allow correlating artefacts to each other and defining the notion of related, refined, and equivalent artefacts. Hermann Ben and co-authors' work \cite{hermannCommunityExpectationsArtifacts2020} in 2020, provided an overview of the current perception and practice of artifact evaluation and the expectations toward artifacts and the process. Besides, Based on community inputs, they also presented suggestions for future development and improvement of artifact evaluations.
\subsection{Empirical Study of Code Repository}
Empirical study of code repository has attracted a lot of attention
\cite{anda2008variability},\cite{kitchenham2020meta},\cite{gonzalez2012reproducibility},\cite{rodriguez2018reproducibility},\cite{cito2016using},\cite{wang2020assessing}. The reproducibility of code repository is a issue gradually attracting more attention. Dacrema Maurizio and co-authors' work \cite{dacremaAreWeReally2019} in 2019 considered 18 algorithms that were presented at top-level research conferences in the last years and found only 7 of them could be reproduced with reasonable effort. Liu Chao and co-authors' work \cite{liuReproducibilityReplicabilityDeep2022}  focused on the reproducibility and replicability of deep learning in Software Engineering. Their statistics showed the urgency of investigating these two factors in SE, where only 10.2\% of the studies investigate any research question to show that their models can address at least one issue of replicability and/or reproducibility and more than 62.6\% of the studies do not even share high-quality source code or complete data to support the reproducibility of their complex models. They concluded it is urgent for the community to provide a long-lasting link to a high-quality reproduction package, enhance DL-based solution stability and convergence, and avoid performance sensitivity on different sampled data.

\jie{add related work on reproducibility in software engineering}
% our work's highlight

Instead of using a script, we manually checked each paper looking for the link to the artefact. 

==> deprecated/IEEE-old/sections_abandoned/result.tex <==
\jie{add connections between our observations and the content from the related works}
\subsection{RQ1 Preparation}
RQ1 describes the general situation in the preparation process of artefacts from five perspectives: whether to establish artefact, storage websites, position of artefact URL in the paper, content of artefact and programming languages.
\subsubsection{RQ1.1 Ratio of Papers with Artefact}
RQ1.1 figures out the changes of ratio of papers with artefact in the past five years.  
Figure \ref{ratioofpaper} shows the number of each conference's papers with and without artefacts from 2017 to 2021. According to our research, the ratio of papers with artefact has increased 59.1\% in 2017 to 79.5\% in 2020 and 68.9\% in 2021. From 2018 to 2019, the ratio of paper with artefacts grew particularly fast. That's because that the software engineering field paid more attention to paper's artefacts in 2019.\draft{Maybe citation here}. In 2021, there are at least 68.9\% of papers in these four conference have corresponding artefacts, which means that everyone's joint efforts are fruitful.

\textbf{Finding 1:} The rapid increment of papers with artefact illustrates that it has become a consensus in the software engineering field that papers should be accompanied by their artefacts. The artefacts of papers help users to verify and apply the research results of papers conveniently, which increasing the application value of papers.



% is listed here as TABLE \ref{THE NUMBER OF PAPERS TAKEN INTO ACCOUNT} .The number of papers in which we find replication package is listed as TABLE \ref{THE NUMBER OF PAPERS WE FIND IN WHICH WE FIND REPLICATION PACKAGES} and the percentage is listed as TABLE \ref{THE PERCENTAGE WE FIND REPLICATION PACKAGES}.

% \begin{table}[htbp]
% \caption{\jie{add RQ number in the title of each table and graph}RQ1: THE NUMBER OF PAPERS TAKEN INTO ACCOUNT}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% &2019&2020&2021&TOTAl\\
% \hline
% ASE&90&92&92&274\\
% \hline
% FSE&74&101&96&271\\
% \hline
% ICSE&108&107&138&353\\
% \hline
% ISSTA&32&45&58&135\\
% \hline
% TOTAL&304&345&384&1033
% \\
% \hline
% \end{tabular}
% \end{center}
% \label{THE NUMBER OF PAPERS TAKEN INTO ACCOUNT}
% \end{table}

% \begin{table}[htbp]
% \caption{THE NUMBER OF PAPERS WE FIND IN WHICH WE FIND REPLICATION PACKAGES}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% &2019&2020&2021&TOTAl\\
% \hline
% ASE&47&83&56&186\\
% \hline
% FSE&52&75&78&205\\
% \hline
% ICSE&65&70&97&232\\
% \hline
% ISSTA&24&33&45&102\\
% \hline
% TOTAL&188&261&276&725\\
% \hline
% \end{tabular}
% \end{center}
% \label{THE NUMBER OF PAPERS WE FIND IN WHICH WE FIND REPLICATION PACKAGES}
% \end{table}

% \begin{table}[htbp]
% \caption{THE PERCENTAGE WE FIND REPLICATION PACKAGES(\%)}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% &2019&2020&2021&ALL\\
% \hline
% ASE&52.22&90.22&60.87&67.88\\
% \hline
% FSE&70.27&74.26&81.25&75.65\\
% \hline
% ICSE&60.19&65.42&70.29&65.72\\
% \hline
% ISSTA&75.00&73.33&77.59&75.56\\
% \hline
% ALL&61.84&75.65&71.88&70.18\\
% \hline
% \end{tabular}
% \end{center}
% \label{THE PERCENTAGE WE FIND REPLICATION PACKAGES}
% \end{table}

% We find with the consciousness of open-source getting popular, although the number of papers these conferences adopt is increasing, both the number of papers containing open-source replication packages and the percentage are in a growth tend on the rise on the whole as well. We can hopefully dream a day when all these papers are born with their link to the replication if it exits, which must decrease the time cost in replicating other researchers' work and focus on our own new work.

\subsubsection{RQ1.2 Storage Website}
RQ1.2 studies the storage websites selected by artefacts. According to our survey, \textit{Github} and  \textit{Zenodo} are top 2 commonly used storage websites of artefacts, occupying 63.7\% and 8.0\% of artefacts respectively. The remaining 28.3\% of artefacts are stored in websites including \draft{gitlab, goo and one drive} or homepages built by themselves. Figure \ref{storagewebsite} shows the ratio of storage websites that artefacts used from 2017 to 2021.  Note that 8.8\% artifacts offer more than one super link or share at more than one website, so these papers will be counted as they offered.


\draft{Here may need to modify}
%29/329 in 2017-2018 
%Besides, although the artefacts stored in above websites, \draft{number\%} of artefacts would like build their homepages to show their contents, which may be in different websites. 
According to our statistics, there are 28.3\% of artefacts built their own homepage to show their contents or share at other websites, among which 25.7\% and 18.4\% of artefacts are build on \textit{github.io} and \textit{google.com} respectively.
\draft{Need further modification}

\begin{figure}[htbp]
	\centering
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pics/1-2/2017_website.png}
        2017
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pics/1-2/2018_website.png}
        2018
	\end{minipage}
	%\qquad
	%让图片换行
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pics/1-2/2019_website.png}
        2019
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pics/1-2/2020_website.png}
        2020
	\end{minipage}
	
	%\qquad
	%让图片换行
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{pics/1-2/2021_website.png}
        2021
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.5\linewidth]{pics/1-2/legend_website.png}
        %legend
	\end{minipage}
\caption{\jie{use bar charts}The ratio of storage websites that artefacts used from 2017 to 2021.}
\label{storagewebsite}
\end{figure}




% \quest{the showcase website and storage website are different...} \draft{According to our survey, \emph{Github, Zenodo, Google Homepage, Github Homepage
% \footnote{Artefacts can be stored in Github and Zenodo. Github HomePage implements the project's Homepage by github.io, but the actual storage website may be somewhere else. Google homepage refers to these having a homepage on Google.}} are four commonly used artefacts storage websites, occupying \draft{number\%}, \draft{number\%}, \draft{number\%}, \draft{number\%} of artefacts respectively.}

In the past five years, Github has been the most commonly used storage website of artefacts. The usage ratio of Github has increased year by year and reach 79.0\% in 2021. It indicates that Github meets the requirements of artefacts storage. In addition, 10.5\% of artefacts are stored in Zenodo in 2021, the usage proportion of which is also increasing year by year. One possible reason is that when the data size of artefacts is too large to be stored in Github with a storage limit of 100M, artefacts would be stored in Zenodo or other websites.\draft{need explain}

\He{Individual files added via the browser IDE are restricted to a file size of 25 MB, while those added via the command line are restricted to 100 MB. Beyond that, GitHub will start to block pushes. Individual repositories, on the other hand, are capped to a maximum of 5 GB.}

\textbf{Finding 2}: Github and Zenodo are the two most commonly used artefacts storage websites, with a usage ratio of 79.0\% and 10.5\% respectively in 2021. In the future, researchers can further study the advantages and disadvantages of these websites when storing artefacts, to build a unified website that is more suitable for artefacts storage management.


\subsubsection{RQ1.3 URL Position}
RQ1.3 explores the position that URL of artefact is provided in a paper, which is a vital problem that the URL of artefact may be ignored if it's given in an inconspicuous position.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/1-3/location.png}
\end{center}
\caption{The ratio of the position that URL of artefact is provided in a paper.}
\label{position}
\end{figure}

Figure \ref{position} illustrates that 44.4\% and 1.2\% of artefacts' URLs are given in the Introduction part and the Abstract part of papers. When we search for URL of artefacts in papers, the two positions are intuitively the most conspicuous. URLs provided in these two positions not only can be searched quickly by keywords, but also are easy to be found while reading. Actually, combined with the data of Figure \ref{position} and the intuition during our experiment, the URLs that appear in the positions with lower proportions are more difficult to find.

\textbf{Finding 3}: A total of 45.6\% of papers provide the URL of artefacts in the Abstract or Introduction. Although authors can put the URL of the artefacts anywhere for the sake of writing, if the artefacts need to be highlighted, providing its URL in the Abstract or Introduction is the most common practice, which help readers to find it easily.

% During our searching for the links for the replication package, we find some interesting phenomenons. Most of authors are likely to contain the name of the tool they develop (if they did so) in the paper.These papers are easier to find the link, because authors always share the links fair and square at the most noticeable ways. For example, some authors are fond of ending the introduction part with their contribution and list the links to their work proudly. According to our estimate, roughly 60\% of the papers which contain open-source replication packages can find the links in the introduction or abstract, especially the end of introduction. Besides these, about 25\% links are found at the end of the paper in a single paragraph. Nearly 10\% of links are found at the middle of the article, usually at the EXPERIMENT part. The rest are hidden in certain corner,such as at the notation of the form. Even some authors leave some text with hyperlinks (For example, ``we share our work \emph{here}'', click \emph{here} will visit their website) This is hard for us to find it. If someone shared their work in this way, we might have ignored it. 

% Authors' habits of how to arrange the links are different widely. Some refer to it just once in their article, while some mention it as many times as they can. Some authors are likely to post their links directly in their article, while some cite it as reference. If the reader can find the links in a short time, how to arrange it doesn't matter. But some articles with a hidden link to their replication packages. This will certainly affect reader's work efficiency. It is necessary to launch a standard about how to share authors' work. We propose a ``\textbf{MOST NOTICEABLE}'' principle here: arrange the link at the end of the introduction part with a single paragraph. We believe every reader can find the link as fast as they can, if he is interested in the article.

\subsubsection{RQ1.4 Content}
\draft{Is there a need to list the artefacts only including introduction as a separate category?}
RQ4 takes care of what content are in the artefacts. According to our investigation, from the aspect of content, there are three kinds of artefact. The first kind of artefact only includes data, results, or a brief introduction, and does not include any code. Such artefact accounts for less than 14.8\% of all artefacts. The second kind of artefact consists of only code without experiment data and the proportion of it has decreased year by year from 2017 to 2021. The third kind of artefact includes both data and code used in the experiments. The proportion of the third kind of artefact has increased from 31.5\% to 45.9\% in the past five years. The number of artefacts that consist of different kinds of content is shown in Figure \ref{content}.
%\draft{data in this figure could not only contain github's.}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/1-4/Figure_4.png}
\end{center}
\caption{The number of artefacts that consist of different kinds of content.}
\label{content}
\end{figure}

To some degree, the first kind of artefacts are not transparent enough to show their experiment process and lack evidence for the reproducibility. Although the code of some artefacts can be simple, it still needs to be shown in the artefacts for users' reference. For the second kind of artefacts, 56.7\% of them implement tools without conducting any experiment using data, so they don't have data in their artefacts. However, there are still 36.9\% of the second kind of artefacts that used experiment data but did not show it. One possible reason for this situation is the need for data confidentiality. The third kind of artefacts not only provide codes that reflect the experimental process, but also provide data for future research. In recent five years, the proportion of the third kind of artefacts has been increasing, which shows that the artefacts community in software engineering field is developing with high quality.
%Java 40 + C/C++ 23 63/111 56.7\%视为implement tool
% python 41/111 36.9\%视为data analysis
\textbf{Finding 4}: The artefacts can be divided into three kinds from the aspect of content. There are 45.9\% of artefacts containing both data and code to ensure the reproducibilty in 2021. It's recommended to provide full data and code in future artefacts if possible.

% Some author just left an introduction on the website, even only a PDF of their article. Some only share their experiment results. These are not what we expect, but they exit and we keep a record.

% Although some can work well without any data, certain repositories are based on necessary data. Some authors just share their code without data, at the meantime some only share their data without code. We made a simple analysis on this and did a statistic on these repositories that are on Github. The result is as follows(TABLE \ref{THE CONTAINING OF REPOSITORIES}). Notice that some authors didn't put the dataset together with their replication repositories. Instead, they offer another link to the data. In this case we consider them as sharing both data and source code.

% \begin{table}[htbp]
% \caption{THE CONTAINING OF REPOSITORIES(\%)}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|}

% \hline
% &only data, result &only code&both data and code&total\\
% &or introduction&&&\\

% \hline
% ASE2019&3&16&10&29\\
% \hline
% ASE2020&6&33&7&46\\
% \hline
% ASE2021&3&25&20&48\\
% \hline
% FSE2019&4&18&11&33\\
% \hline
% FSE2020&5&30&10&45\\
% \hline
% FSE2021&12&17&35&64\\
% \hline
% ICSE2019&7&21&15&43\\
% \hline
% ICSE2020&6&28&8&42\\
% \hline
% ICSE2021&16&23&32&71\\
% \hline
% ISSTA2019&2&5&4&11\\
% \hline
% ISSTA2020&2&16&6&24\\
% \hline
% ISSTA2021&7&15&13&35\\
% \hline
% 2019&16&60&40&116\\
% percentage&16.0\%&50.4\%&33.6\%&\\
% \hline
% 2020&19&107&31&157\\
% percentage&12.1\%&68.2\%&19.7\%&\\
% \hline
% 2021&38&80&100&218\\
% percentage&17.4\%&36.7\%&45.9\%&\\
% \hline
% total&73&247&171&491\\
% percentage&14.9\%&50.3\%&34.8\%&\\
% \hline
% \end{tabular}
% \end{center}
% \label{THE CONTAINING OF REPOSITORIES}
% \end{table}

% As the statistics show, the repositories without code are only a few, and most of them contain them. But there are many repositories that only have code and no data. In the process of analyzing statistics, we quickly browsed some repositories and found that most of them are some kind of tools developed. There are also some data analysts who share their analysis scripts but do not publish the data. At the same time, we analyzed the repositories containing both code and data, and found that many of them are related to data analysis. In addition, this section contains some repositories related to machine learning. In particular, we noticed that repositories containing data generally use Python.

\subsubsection{RQ1.5 Programming Language}
RQ1.5 focuses on programming languages used in artefacts. As Figure \ref{progamminglanguage} shows, Java, Python and C/C++ are the most used programming languages, accounting for 29.8\%, 51.1\% and 15.4\% respectively. At the same time, other programming languages, including R, Go, Pascal, C\#, F\#, JavaScript, Matlab, Ocaml, Scala, Rust, CSS, HTML, PHP, Kotlin, LLVM, etc, are also used. What's more, 81.0\% of artefacts use multiple programming languages.
%and account for \draft{number\%} in total.

\quest{need discuss}
\He{I insist on not offering a percentage of the  general others because just making subtract directly is unscientific and here need to offer the percentage of each language but it doesn't deserve and take much both space and effort}

\draft{we should count all the website not only Github, or find a convincing explanation....}

\He{only github offer a percentage of usage of each program language,I have no idea about how to analyze this on the repositories from other website}

\draft{Here I think it is necessary to clarify how these languages are counted. Are all languages used by an artefact involved in the count?}


It is convincing that Python and Java have been the two most used programming languages for the past five years. Java is often used to development tools and Python is becoming more and more popular with the growing need of data processing and machine learning. Therefore, these two languages are important for the current and future artefacts.


\draft{What's more, 81.0\% of artefacts use multiple programming languages. Among the artefacts that use only one programming languages, \draft{number\%} and \draft{number\%} of them use Python and Java respectively, and the remaining \draft{number\%} use other programming languages including C\#, \draft{Here may need to modify}.}
%2017-2018 31/163 single
\He{here need to decide whether it's necessary to discuss these here. If the paper is long enough, I intend to delete the up paragraph}



\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{pics/1-5/Figure_5.png}
\end{center}
\caption{The number of the programming language used in artefacts.\jie{revise, detaileds suggestions in wechat group}}
\label{progamminglanguage}
\end{figure}


In addition, the proportion of various programming languages used in each artefact are recorded in preparation for further selection of artefacts suitable for detecting code smells.

\textbf{Finding 5}: Python and Java are two most used programming languages in artefacts, accounting for 51.1\% and  29.8\% . And \draft{number\%} of artefacts use more than one kind of programming language.

% \begin{table}[htbp]
% \caption{THE LANGUAGE USED IN THESE REPOSITORIES}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|}

% \hline
% &Java&Python&C/C++&total on Github\\
% \hline
% ASE2019&11&15&8&29\\
% \hline
% ASE2020&7&28&6&46\\
% \hline
% ASE2021&7&30&6&48\\
% \hline
% FSE2019&15&14&5&33\\
% \hline
% FSE2020&13&30&7&45\\
% \hline
% FSE2021&9&41&9&64\\
% \hline
% ICSE2019&16&15&5&43\\
% \hline
% ICSE2020&7&18&4&42\\
% \hline
% ICSE2021&17&33&8&71\\
% \hline
% ISSTA2019&3&7&1&11\\
% \hline
% ISSTA2020&7&16&6&24\\
% \hline
% ISSTA2021&6&20&4&35\\
% \hline
% 2019&45&51&19&116\\
% percentage&38.79\%&43.97\%&16.38\%&\\
% \hline
% 2020&34&92&23&157\\
% percentage&21.66\%&58.60\%&14.65\%&\\
% \hline
% 2021&39&124&27&218\\
% percentage&17.89\%&56.88\%&12.39\%&\\
% \hline
% total&118&267&69&491\\
% percentage&24.03\%&54.38\%&14.05\%&\\
% \hline
% \end{tabular}
% \end{center}
% \label{THE LANGUAGE USED IN THESE REPOSITORIES}
% \end{table}

% According to the statistics, Java and Python are the most widely used languages in these repositories. Java is often used to development tools; while Python is becoming more and more popular with the growing need to process data, there are many mature packages available for easy use. Further inspection found that in repositories that use Java or Python, their proportion is often high, and they are used as the main hospital. As a comparison, although C/C++ is also frequently used, the proportion is very low in many places, just to implement some components or use it with other languages when there are other specific requirements. And this is not conducive to our more in-depth analysis of it. At the same time, because the testing tools are easily interfered, the low proportion of language will make analysis difficult and even cause errors. Therefore, considering the above considerations, in further research, we select repositories that use Java or Python and account for more than 10\% of the repositories for codesmell analysis.

\begin{tcolorbox}
\textbf{\underline{Answer to RQ1:}} 
From 2017 to 2021, artefacts of papers have received more and more attention. The ratio of papers with artefact is increased from 59.1\% in 2017 to 79.5\% in 2020 and 68.9\% in 2021. 45.6\% of the papers consider artefacts as an vital contribution and highlight the URL of artefacts in the Abstract or Introduction section. The proportion of artefacts containing both data and code has increased during these years, and reaches 45.9\% in 2021. Besides, 63.7\% of artefacts are stored on github. The data of artefacts would be stored in various websites if its data size exceeds the storage limitation of github. Using by more than 51.1\% of artefacts, Python is the most used programming language.
\end{tcolorbox}

% Over the past three years, open source implementations and data contributions in papers have received increasing attention. Many enthusiastically placed their open source links prominently in the article. Here we present our proposal: MOST NOTICEABLE. Due to its ease of use and high acceptance, Github is attracting more and more developers to put their repositories on it for others to use. For users, getting the right code and data is almost equally important. We call for sharing code along with data whenever possible, if your project requires it. It has gradually become a trend to choose the corresponding programming language according to the required functions.

\input{sections/RQ2}

\input{sections/RQ3}

\input{sections/RQ4}

==> deprecated/body.tex <==

\section{Introduction}


Artifacts of publications play a vital role in research\footnote{In this paper, following previous work (\cite{ChristopherTimperley2021}),
we define an artifact as ``any external materials or information provided in conjunction with a research paper via a link''. }.
Artifacts improve the understanding and provide supportive evidence for the claims in a research paper.
They also facilitate code and data reuse and allow for future extension, improvement, and comparison (\cite{ChristopherTimperley2021}). 
Artifacts have gotten more and more attention from the research community since 2016, after a crisis of reproducibility was made open to the public by a Nature’s survey in which more than 1,500 researchers revealed having trouble reproducing previous research results (\cite{baker20161}).
%\footnote{Chatgpt~\cite{ChatGPT} participated only in spelling and grammar checking and writing polish for this paper.}

Software Engineering (SE) community is one of the research communities that have put substantial effort in encouraging open-source artifacts.
Artifact evaluation has become a regular process for software engineering conferences (\cite{hermannCommunityExpectationsArtifacts2020}).
Reproducibility and transparency with artifacts have become one of the key review criteria for top-tier conferences such as 
% ICSE 2022 
\cite{icsereviewguideline} 
and 
% FSE 2022
\cite{fsecfp}.
% The Open Science Policy in the call-for-papers of FSE 2022 mentioned that 
% ``\emph{Openness in science is key to fostering scientific progress via transparency, reproducibility, and replicability.}''
These efforts have yielded a pleasing increase in the prevalence of open-source artifacts.
As shown in Figure~\ref{fig:ratioofpaper},
the ratio of top-tier publications (ICSE, FSE, ASE, and ISSTA) with artifacts has increased from 60.1\% to 81.1\% from 2017 to 2022 according to our analysis.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.48\textwidth]{images/figure_1.pdf}
\end{center}
\vspace{-5mm}
\caption{Number and ratio of top-tier publications with and without artifacts from 2017 to 2022.}
\label{fig:ratioofpaper}
\end{figure}

Given the importance of artifacts in SE community, some pioneering efforts have been made.
% Hermann et al. 
\cite{hermannCommunityExpectationsArtifacts2020} pointed out the community expectations for artifacts by collecting comments from program committee members. 
% Timperley et al. 
\cite{ChristopherTimperley2021} explored the general situation of the artifact community from 2014 to 2018 and raised some notable recommendations. 
% Shriram et al. 
\cite{krishnamurthi2015real} not only emphasized the importance of repeatability and artifact evaluation but also regarded repeatability as \emph{the real software crisis}.

Despite the efforts from conference organizers and the existing research on the expectations of artifact evaluation, it is unclear how well the current practice of research artifacts performs.
%the current status and trends of artifact practices, maintenance, popularity, and quality in the software engineering community, remain unclear.
% Aristotle said: ``Knowing yourself is the beginning of all wisdom.''
Investigation on the research artifacts in SE publications can be helpful to 
understand the strengths and weaknesses of artifact preparation and be open to a range of measures to improve them.
%\draft{need reorganising, a reviewer point that the reason is unadequate}

To this end, this paper presents an empirical study on the status and trends of research artifacts in software engineering publications in the past six years (from 2017 to 2022).
\revise{
We study the data from 2017 onwards due to the reproducibility crisis that emerged in 2016 (\cite{baker20161}) and its significant impact on the field of software engineering. 
The SE community has witnessed a considerable increase in the concern for the reproducibility of publications since 2017.
Therefore, the data from this time frame can accurately illustrate the current status and trends of SE artifacts.
}
In particular, we focus on four aspects of artifacts, including 
(1) \textit{common practices}: the types of uploading repositories, programming languages, and the locations in a paper where the links are provided;
(2) \textit{maintenance}: the validity of the provided links and the maintenance time distribution of artifacts;
(3) \textit{popularity}: the star number distribution and the characteristics of top-starred artifacts;
(4) \textit{quality}: the content of documentation and the existence of code smells.

\revise{These four aspects illuminate common procedures, durability issues, potential impact, and usability concerns, offering a comprehensive perspective on artifacts within the software engineering community.}
Note that we aim to overview the status and trends of SE artifacts in this single paper as much as possible. 
Despite we choose the four most representative aspects, there are still many interesting points worth further study. 
We hope that our work can arouse more interest from the community to work in this direction and provide more systematic and deep studies on real-world artifacts.

% There are certainly many interesting points to dig deep into in other aspects.  
% It is impossible for us to cover them all in one single paper. 
% Instead of providing a deep and comprehensive analysis for all possible aspects, this paper aims to provide an overview of the current status and trends of artifacts in the SE community and focus on the most intuitive aspects. We hope that our work can arouse more interest from the community to work in this direction and provide more systematic and deep studies.

% \draft{I agree that not all aspects can be evaluated, but an explanation of why the selected aspects are the most important for the community and why they help with the arc in the introduction, coming down to Aristotle's quote, is missing. Currently, it looks like these aspects are the easiest ones to to assess, not the most important ones.
% }

\revise{
To obtain the dataset for analysis, we carefully select the venues to reach the frontier status of artifacts in SE research.
According to the top-tier venue list of SE provided by the \cite{csranking}, we choose the research track of the four software engineering conferences: {International Conference on Automated Software Engineering} (ASE), {ACM SIGSOFT Symposium on the Foundation of Software Engineering/ European Software Engineering Conference} (FSE), {International Conference on Software Engineering} (ICSE), and {International Symposium on Software Testing and Analysis} (ISSTA). 
These conferences are well recognized to be the top-tier four SE conferences (\cite{kim2018precise,kochhar2016practitioners}), and are expected to represent the best practices of research artifacts in the SE community.
We believe that artifacts in these four conferences represent the cutting-edge status and trends in software engineering.
}

\revise{
We focus on publications with a minimum of 6 pages, as they are considered to reflect a more mature status compared to shorter papers.
In total, our dataset comprises 2,196 papers. 
We then employ a labor-intensive approach to extract artifact URLs from these publications, resulting in the identification of 1,487 papers offering research artifacts.
}

Our analysis of these artifacts yields the following primary observations and findings.

In terms of \textit{common practices},
(1) An increasing proportion of SE publications disclosed their artifacts in the past six years (from 60.5\% in 2017 to 78.3\% in 2022), revealing growing recognition of the value of open research artifacts.
(2) Though most SE conferences now explicitly recommend Zenodo over GitHub as an artifact repository platform, the majority (64.2\% in 2022) of researchers choose GitHub for artifacts, likely due to its ease of maintenance and familiarity.
The ratio of Zenodo adoption has increased from 0.0\% to 16.0\% over the past six years. 
(3) Python has overtaken Java to become the most widely used language in artifacts (61.1\% in 2022), calling for more research on quality metrics and automatic examination approaches towards Python, similar to the code smell towards Java.

Regarding \textit{maintenance},
(4) The proportion of link rot\footnote{Due to inactive maintenance, artifacts may become unavailable over time. This phenomenon is called \emph{link rot} (\cite{wwwFetterlyMNW03}), which means that the provided URLs cease to point to their originally targeted artifacts.} raises over time, from 4.8\% in 2022 to 29.8\% in 2017. 
The ratios of link rot on GitHub and dedicated archiving platforms like Zenodo are merely 6.4\% and 7.1\%, suggesting special attention on the long-term availability of artifacts stored outside commonly used artifact service platforms during the review process.
\revise{
Researchers can leverage tools like the Wayback Machine (\cite{wayback_machine}), robust links (\cite{jones2021robustifying}), or similar technologies to guarantee the enduring availability of their artifacts.
}
(5) At least half of artifacts require ongoing updates after conferences, highlighting an advantage of GitHub over archiving platforms like Zenodo. Thus, conferences should not blanket recommend against using GitHub but rather should guide researchers to choose the suitable platform for their specific artifacts. 
\revise{
Additionally, Zenodo can now track updates from GitHub, facilitating collaboration between the two platforms for artifact publication. Researchers may also consider Software Heritage as a durable and citable code archive that considers subsequent commits.
}

As for \textit{popularity}, 
(6) Most GitHub artifacts receive limited attention, with 65.0\% attracting no more than 10 stars. Though artifact star counts inaccurately gauge popularity, they indicate most software engineering artifacts lack real-world adoption and impact. We believe that rather than only supplement papers, more artifacts should aim to shape real-world applications.
% Star numbers and time did not show a clear correlation.

Considering \textit{quality}, 
(7) Over 96\% of projects trigger code smell alerts mainly for code convention rather than functional issues, indicating that code smell detection seems insufficient to accurately assess code quality for artifacts. Research on tailored metrics focused specifically on the code quality of artifacts is necessary.

% On average, code smell alert messages appear in 99.2\% of Python projects and 95.0\% of Java projects. 
% However, the majority of code smell alert messages are related to code convention rather than functional issues, indicating that functionality is not the main quality concern. 

% Artifacts documentation quality is fair and has not changed much in recent years. 

\revise{
In summary, this paper makes the following contributions:
\begin{itemize}
    \item We conduct an empirical study on the current status and trends of artifacts in the SE community, which reflects the overall situation.
    % \item We compare the status in the past six years (2017 to 2022) with the previous work (\cite{ChristopherTimperley2021,hermannCommunityExpectationsArtifacts2020}) and current criteria (\cite{acmguidelines}) to present some of the key problems that need to be addressed in artifact community of SE.
    \item We present a comprehensive analysis of our empirical results and provide suggestions for different stakeholders to enhance the artifacts practice.
    \item We publicly release our data, scripts, and results for further study.
\end{itemize}
}

The rest of this paper is organized as follows.
Section~\ref{sec:methodology} describes the methodology of our study. 
Section~\ref{sec:Results} illustrates the experimental results and findings. 
Section~\ref{sec:Discussion} discusses our suggestion and threats to validity. 
Section~\ref{sec:Related Work} describes the related work. 
Section~\ref{sec:Conclusion} concludes the paper. 
Section~\ref{Data Availability} provides our artifact.
\section{Methodology}
\label{sec:methodology}

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=0.65\textwidth]{images/methodology.pdf}
\end{center}
\caption{\revise{The overview of our methodology.}}
\label{fig:methodology}
\end{figure*}

\revise{
This section introduces our methodology (Figure~\ref{fig:methodology}), including research questions,
venue selection,
paper and artifact collection process,
and the information extraction details.
}

\subsection{Research Questions}

To elucidate the status and trends of SE artifacts, we aim to answer the following four research questions (RQs). 

\emph{RQ1. Common practices:} What are the common practices for software engineering researchers to prepare their artifacts? 

\emph{RQ2. Maintenance:} How well do researchers maintain their artifacts?

\emph{RQ3. Popularity:} How is the popularity of existing artifacts and what are the characteristics of top-starred artifacts?

\emph{RQ4. Quality:} How is the quality of the artifacts in terms of the documentation quality and code smells?

\revise{
Our four RQs encompass four crucial aspects of artifacts, each offering valuable insights into the current state of SE artifacts.

First, RQ1 aims to understand common practices in artifact preparation, serving as a foundation for enhancing the process. By addressing RQ1, we can identify gaps and potential areas for improvement in terms of discoverability, accessibility, and ease of setup.

Second, artifact maintenance directly impacts their longevity and usefulness over time. RQ2 examines the significance of maintenance and investigates existing strategies and potential enhancements.
We specifically focus on link rot, a widely acknowledged phenomenon that significantly undermines the reproducibility of artifacts (\cite{d2015urls,sanderson2011analyzing,klein2014scholarly}).

Third, the popularity of artifacts provides insights into their adoption and usage within the software engineering community, which helps identify artifacts that have made a significant impact and garnered attention from researchers and practitioners.
RQ3 reveals the popularity of current artifacts and provides recommendations for promoting their influence and sharing.

Fourth, ensuring artifact quality is fundamental for reproducibility and reuse. 
RQ4 focuses on documentation (\cite{SoftwareDocumentation2019}) and code smell (\cite{santos2018systematic}) as metrics for quality, which are widely recognized and established measures for evaluating artifacts in the software engineering community.

On the one hand, the artifact quality heavily depends on the documentation quality, which impacts the clarity, completeness, and ease of reproduction of an artifact.
Clear and well-documented artifacts facilitate reproducibility and allow other researchers to build upon existing work effectively. 

On the other hand, code plays a vital role in the SE community and makes up a significant part of SE artifacts. 
Code smells can affect the readability, maintainability, and extensibility of code, which ultimately impacts the quality of the research artifacts. 
By analyzing code smells, we can identify potential design issues or violations of good programming practices within artifacts, and contribute to enhancing the code quality of the artifacts.
}

By addressing these four research questions, we aim to provide a comprehensive understanding of the status and trends of research artifacts in SE.
For ease of presentation, we use Table~\ref{RQs} to demonstrate the content of each RQ.



\begin{table*}[h!]
\caption{Research questions of our study. Each research question is answered from different perspectives.
}
\begin{center}
\resizebox{0.96\textwidth}{!}{\

\begin{tabular}{l|ll}
\toprule
Research Questions & Content & Explanation\\
\midrule
\multirow{3}*{RQ1: Common practices}&Storage websites&What sites or service do researchers use to upload their artifacts?\\
&URL location \&  format&Where in the paper and how do researchers provide their artifacts URL?\\
&Programming language& How does usage of the most popular programming languages vary among artifacts?\\
\midrule
\multirow{2}*{RQ2: Maintenance}
&invalid URLs& How many artifact URLs have become invalid?\\
% \cline{2-3}
&Last update time& How does the maintenance of artifacts by researchers relate to conference progress?\\
\midrule
\multirow{2}*{RQ3: Popularity}& Star situation &How many stars do artifacts have?\\
% \cline{2-3}
&Characteristics& What are the characteristics of top-starred artifacts?\\
\midrule
\multirow{2}*{RQ4: Quality}&Documentation& How is the quality of the documentation provided by researchers?\\
&Code smell& What are the common code smells in the artifacts?\\

\bottomrule

\end{tabular}}
\label{RQs}
\end{center}
\end{table*}


\revise{
\subsection{Venue Selection}

In the field of software engineering, novel results tend to be published through \emph{conferences}, while their incorporation into \emph{journals} may not always be guaranteed or immediate.
Consequently, following previous work (\cite{abou2022software}), 
we concentrate on conferences, which we posit to be a reliable representation of the latest research trends in software engineering during a specific time frame.

To examine the latest advancements in SE artifacts for each year, we focus on publications in the software engineering category of~\cite{csranking}. 
The CS Rankings is a widely acknowledged website that provides an entirely metrics-based ranking system for computer science, which selects the most prestigious publication venues in each area of computer science, including software engineering.
Specifically, we consider ICSE, FSE, ASE, and ISSTA, which are widely recognized as top-tier venues in the field of SE (\cite{kim2018precise,kochhar2016practitioners}), thereby being a good start for the community to understand the best practices in research artifacts.

Overall, we consider these conferences to showcase state-of-the-art research in software engineering, with their associated artifacts capturing the latest advancements in the field each year.
}

\revise{
Additionally, we study the data from 2017 onwards due to the reproducibility crisis that emerged in 2016 (\cite{baker20161}) and its significant impact on the field of software engineering. 
The SE community has witnessed a considerable increase in the concern for the reproducibility of publications since 2017.
Consequently, the data from this time frame can accurately illustrate the current status and trends of SE artifacts.
}


\subsection{Collection of Papers and Artifacts}
\label{sec:method:collection}




\revise{

To obtain the paper list, we utilize the \cite{dblp} bibliography to search for papers and download them using their DOIs.
\cite{dblp} is a widely-used computer science bibliography, ensuring the comprehensiveness of our dataset without omissions.

We further refine our dataset by excluding short papers, following \cite{khalil2022general}.
Full papers, which typically present more mature and established results, ensure a more comprehensive representation of the frontier state.
To achieve this criterion, we filter out papers with less than 6 pages, based on DBLP metadata.
 
As a result, we download 2,196 full papers from the research track (i.e., the main track) of four top-tier conferences in the SE community, including ASE, FSE, ICSE, and ISSTA, from 2017 to 2022.
}
% We choose these four conferences because they are widely acknowledged to be the top four SE conferences (\cite{kim2018precise,kochhar2016practitioners}),

\revise{
We try our best effort to obtain artifact URLs in papers.
Specifically, we first define a set of search keywords to help us quickly locate the URL, including  ``available'', ``https'', ``replication'', ``reproducibility'', ``code'', ``data'' and some other similar words. 
Then, we conduct a manual search in each paper for artifact URLs by looking for the above keywords. 
If we do not find any URLs during this search, we browse the paper to check if any URLs are mentioned as artifacts again.
Once we have identified these URLs, we manually verify if they correspond to the respective paper.
}

\revise{
We improve the accuracy of the annotation results by double-checking.
In detail, two authors of this paper independently annotate the URLs for each paper and cross-check them once all annotations are completed. 
In case of conflicts, we hold discussions to reach a consensus. 
}

\revise{Based on our parsing methods, we find 1,487 papers containing artifact URLs.
Table~\ref{tab:detail} shows the results of our collection of papers and artifacts for the four top-tier SE venues from 2017--2022.
Each cell presents the number of papers with artifacts followed by the total number of papers, with the corresponding percentage of papers with artifacts provided in parentheses.
We also present the growing trends of papers with artifacts in Figure~\ref{fig:trends}.
}

\begin{table*}[h!]
\caption{
\revise{
Results of papers with artifacts and the total number of papers.
}
}
\begin{center}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
\toprule
Venue & 2017 & 2018 & 2019 & 2020 & 2021 & 2022 & Total \\
\midrule
ASE & 67/105 (63.8\%) & 51/80 (63.7\%) & 46/84 (54.8\%) & 61/93 (65.6\%) & 56/85 (65.9\%) & 91/116 (78.4\%) & 372/563 (66.1\%) \\
FSE & 47/90 (52.2\%) & 49/75 (65.3\%) & 56/95 (58.9\%) & 78/125 (62.4\%) & 87/120 (72.5\%) & 91/133 (68.4\%) & 408/638 (63.9\%) \\
ICSE & 45/68 (66.2\%) & 65/105 (61.9\%) & 66/109 (60.6\%) & 87/129 (67.4\%) & 97/138 (70.3\%) & 164/197 (83.2\%) & 524/746 (70.2\%) \\
ISSTA & 19/31 (61.3\%) & 21/31 (67.7\%) & 24/32 (75.0\%) & 31/43 (72.1\%) & 37/51 (72.5\%) & 51/61 (83.6\%) & 183/249 (73.5\%) \\
Total & 178/294 (60.5\%) & 186/291 (63.9\%) & 192/320 (60.0\%) & 257/390 (65.9\%) & 277/394 (70.3\%) & 397/507 (78.3\%) & 1487/2196 (67.7\%) \\
\bottomrule
\end{tabular}}
\end{center}
\label{tab:detail}
\end{table*}

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=0.95\textwidth]{images/figure_8.pdf}
\end{center}
\vspace{-5mm}
\caption{
\revise{Trends of papers with artifacts.}
}
\label{fig:trends}
\end{figure*}

\subsection{Information Extraction}

To answer the research questions, we extract the following information from collected papers and artifacts.

\subsubsection{Paper Examination}

\revise{
When obtaining the paper list, we gain the publication year, venue, and title of papers from DBLP.

During the process of manually exploring the artifact URL, we record the location and format of artifact URLs for papers in which we find artifacts.
Typically, we record the URL location and format where we first find the URL in a paper, which can be considered the most prominent placement of the URL.
We categorize the \textbf{URL location} into title, abstract, introduction, conclusion, and other sections because the first four sections are common to all papers.
We also mark the \textbf{URL format} that researchers choose to provide the URL, which is classified into footnote, reference, in-text, and hyperlink. 
}

\subsubsection{Artifact Examination}

We examine each artifact to collect the information for the content we list in Table~\ref{RQs}.

\noindent\textbf{Storage websites:}
We classify the storage websites of our collected artifacts into GitHub\footnote{\url{https://github.com/}}, Zenodo\footnote{
\url{https://zenodo.org/.} Zenodo is a general-purpose open repository for researchers to deposit any form of research-related digital artifacts. }, self-built homepages (with support from GitHub, Google, or other websites), and others (primarily temporary data drives).
\revise{
There are 4.6\% of papers utilizing multiple types of storage websites.
We document all the employed storage websites for each paper.
}

\noindent\textbf{Programming languages:} 
We observe that the storage website of most artifacts is GitHub, which will display the proportion of programming languages used in artifacts.\footnote{Linguist is used on GitHub.com to detect blob languages, ignore binary or vendored files, suppress generated files in diffs, and generate language breakdown graphs. For more information of linguist, check \url{https://github.com/github/linguist} .} 
By leveraging the GitHub APIs, we identify the programming languages utilized by GitHub artifacts, yielding 794 artifacts with the corresponding programming languages.

% We notice that Python, Java, and C/C++ are the top three popular programming languages in artifacts, which is consistent with HelloGitHub's statistics\footnote{\url{https://hellogithub.com/report/tiobe/}}. 
% Therefore, we focus on the three languages and study how the usage ratio changes. 
% Other programming languages, including R, Go, Pascal, C\#, F\#, JavaScript, Matlab, Ocaml, Scala, Rust, CSS, HTML, PHP, Kotlin, LLVM, are also used in artifacts.

\noindent\textbf{Last update time:} Utilizing Github APIs, we record the latest update time for 901 Github artifacts. 
The latest update can be regarded as the most recent modification made to an artifact, specifically the time of the last push on GitHub.

Next, we manually search the web for the important dates of conferences each year, including the paper submission deadline, paper notification time, camera-ready deadline, and conference time.
We record the ratio of artifacts that get updated after each deadline.

\noindent\textbf{Invalid URLs:} 
%Due to inactive maintenance, artifacts may become unavailable over time. This phenomenon is called \emph{link rot} \cite{wwwFetterlyMNW03}, which means that the provided URLs cease to point to their originally targeted artifacts.
We record whether the URLs of artifacts provided in papers are valid or not by manually accessing each URL.

\noindent\textbf{Star number:}
``Star'' on GitHub can be described as a form of social endorsement or signaling. 
When starring a repository, the repository will be added to the starred repository list of users, which serves as a personal bookmark and can also indicate to other users that the repository is worth checking out.
As more users star a repository, it becomes more visible within the GitHub community. 
The number of stars a repository has can serve as social proof of its usefulness or interest to potential users, demonstrating that it has been evaluated and endorsed by others.

Therefore, the number of a repository's stars is strongly linked with its overall popularity. In total, we record 783 artifacts with their star numbers through the GitHub API.


\noindent\textbf{Characteristics of top-starred artifacts:}

\revise{
According to the distribution of stars, only 3.7\% of GitHub artifacts boast more than 100 stars. 
Therefore, we consider these artifacts as top-starred and explore their characteristics. 
Employing this criterion, we identify a total of 33 top-starred artifacts.
In addition to the preceding collected information, we record the documentation quality, executability, number of forks and issues, as well as the latest update time associated with these top-starred artifacts.
}

\noindent\textbf{Documentation:} 

\revise{
When examining an artifact on GitHub, we record the documentation quality by manually checking the README file in the artifact. 
Referring to \cite{SoftwareDocumentation2019}, we selected six simple and feasible criteria to measure artifacts. Each criterion is marked by yes or no.

The specific criteria are :
(1) Completeness: Whether the README contains the system version, software, and library environment requirements. \footnote{If the README says ``Please check this file for this information,'' we'll check that file and consider it part of the README. If this file meets the criteria, we also consider the README file to meet the criteria. Unless otherwise stated, the following will follow this principle.}
(2) Structure: Whether the README describes the file structure of the artifact, no matter whether it is accurate to each file or roughly what is in each folder.
(3) Usability: Whether the README contains how to use the artifact.
(4) Example: Whether the README contains any use examples or display of the effect when used.
(5) Certificate: Whether the README states this artifact has a certificate or a certificate can be found along with the README. Furthermore, we record the type of the certificate.
(6) Contact: Whether the README contains the researchers' contact information or the researchers' reply on the topic. \footnote{Notice that on GitHub, the owner of every repository can be found. However, we believe that only the two ways mentioned above reflect the positive willingness of researchers to contact. So these are the only two ways that we would consider satisfying this criterion.} 

Considering the substantial manual effort required for this examination, and recognizing that it is just one aspect of our overall study, we focus specifically on GitHub artifacts from the ICSE spanning the years 2017 to 2022. Given that ICSE features a larger number of papers compared to the other three venues, we consider this subset to be representative enough for our documentation analysis.
}

\noindent\textbf{Code smells:}

Code that follows a consistent style is much easier to read, which can help others to understand, maintain, and reuse the artifact more efficiently. 
So the code style is crucial to the overall quality of artifacts.

According to the statistics mentioned earlier in ``Programming languages'', Python and Java are the two most used programming languages that dominate the artifacts we collect.
In addition, these languages are supported by well-established code quality metrics (i.e. code smell) and detection tools.
Therefore, we focus on Python and Java artifacts to explore the prevalence of code smell. 

We use \cite{pylint} to collect the code smell information for Python, and \cite{pmd} to collect the information for Java.
We choose these two tools due to their popularity and reliability.
The GitHub repository of Pylint and PMD has over 4.1k stars and 3.9k stars, respectively.
In particular, the Pylint is based on the 
% PEP8
\cite{PEP8}, a style guide for Python code. 

% \revise{
% Due to the limitations of code smell detection tools in generating comprehensive reports for small code volumes, we exclude artifacts where the Python or Java usage ratio is below a certain threshold (10\%) to ensure accurate assessment of code quality.
% Additionally, artifacts utilizing less than 10\% of Python/Java code cannot be accurately assessed for code quality based solely on Python/Java code smells. 
% As a result, we have 407 Python artifacts and 257 Java artifacts as our subjects for the analysis of code smells.
% }

\revise{
Due to the limitation of the GitHub API, we can only retrieve the primary programming languages for each repository. 
Therefore, We detect code smells for artifacts coded in "Python" or "Java" based on the information provided by the GitHub API. 
To avoid potential infinite loops within a single artifact, we set a time limit of 60 seconds for each detection, which is typically adequate for the majority of artifacts.
As a result, we successfully perform code smell detection on 268 Python artifacts and 144 Java artifacts.
}

% \subsection{Analysis of Results}
% We use percent stacked column charts\cite{percentstackedcolumnchart} to demonstrate the distribution and trends for storage websites, content, programming languages, documentation, and invalid URLs of artifacts. Pie charts are used to demonstrate the distribution of those characteristics for which time is more likely to be irrelevant.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}
\label{sec:Results}
This section introduces the results of our study.
For each research question, we present the analysis results and discuss our observations and conclusions.


\subsection{RQ1: Common Practices}
RQ1 aims to understand the common practices of SE researchers when preparing artifacts. To answer RQ1, we classify the collected artifacts according to the categories in each aspect (i.e., storage website, URL location, and programming languages), and 
analyze the distribution of the artifacts.

\subsubsection{Storage Website}

Figure~\ref{storagewebsite} shows the detailed results of storage websites of artifacts. 
We observe that GitHub is the most widely used website and has gained more and more adoption since 2017.
In 2022, 64.2\% of the artifacts are stored in GitHub repositories.

The second most popular website is Zenodo.
The ratio of artifacts on Zenodo has increased dramatically from 0.0\% to 16.0\% from 2017 to 2022.
Zenodo is a dedicated platform for sharing artifacts, providing researchers with a seamless and anonymous process for uploading their artifacts.
Besides, researchers' operations are recorded on Zenodo. 
When researchers update their artifact, a URL for an artifact on Zenodo will show the original artifact with a hint that there is a newer version, while a URL for an artifact on GitHub will just show the newest version without the availability of the original version.
In addition, every upload in Zenodo is assigned a Digital Object Identifier (DOI), to make the artifact citable and trackable. 
Our observation that Zenodo is getting more adoption aligns with the ``Submission and Reviewing Guidelines'' of the FSE 2021 Artifact Evaluation track (\cite{fsereviewguideline}) (abbreviated as ``FSE21 guideline'' in the remaining part of this paper)
which ``strongly recommends relying on services like Zenodo to archive repositories''.
The open science policy of ICSE 2021 to 2023 also suggests authors archive artifacts on preserved digital repositories such as Zenodo.
As a result, the ratio of artifacts on Zenodo in 2022 (16.0\%) is almost twice as much as it was in 2021 (9.0\%).

The remaining artifacts are published on individual/ institutional websites or temporary drives (e.g., Dropbox, Google Drive, GitLab, and OneDrive). The ratio of these artifacts has decreased from 55.6\% to 19.7\% in the past six years.
The decrease in the ratio of artifacts on individual/institutional websites or temporary drives is also a positive change because these websites are prone to changes and are regarded as non-persistent (\cite{fsereviewguideline}). Besides, These artifacts face more Link Rot as shown in RQ2.2.

% \jie{mention ICSE 2023 open-science policy:Just a reminder that this year ICSE recommends a separate section of ``Data availability'' in the end of the paper and GitHub is not recommended for the artifact repository (Zendo is recommended).}


Archived on preserved digital repositories such as \url{zenodo.org}, \url{figshare.com}, \url{www.softwareheritage.org}, \url{osf.io}, or institutional repositories such as GitHub, GitLab, and similar services have version management and update time record capabilities. 
Researchers can do vigorous content management on their artifacts under the protection of historical versions without worrying about an error of operation and the coming problems that cause the devastation are difficult or impossible to recover from. For the visitors of the artifact, they can find the specific version or the specific files uploaded at a certain time, instead of just the newest version of the whole artifact. Such advantages are not possessed by Personal or institutional websites, consumer cloud storage such as Dropbox, or services such as \url{Academia.edu} and \url{Researchgate.net}.


\begin{findingbox}{
The majority  (64.2\% in 2022) of publications still upload their artifacts on GitHub, even though services for version control systems are not recommended in some conferences (\cite{icse23policy}).
The ratio of Zenodo adoption has increased \textbf{from 0.0\% to 16.0\%} over the past six years. Due to its strengths and the conferences' recommendations, the usage ratio of Zenodo has been and will continue to grow rapidly.
}\end{findingbox}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.48\textwidth]{images/figure_2.pdf}
\end{center}
\vspace{-5mm}
\caption{Distribution and trend of storage website adoption for SE artifacts from 2017 to 2022.}
\label{storagewebsite}
\end{figure}

\subsubsection{Programming Language}
This part focuses on the programming languages contained in the artifacts. 
The programming language is a core characteristic of most SE artifacts, though not all the artifacts contain code. 
Figure~\ref{progamminglanguage} shows the ratio of artifacts with the three most widely adopted programming languages: Python, Java, and C/C++.

We observe that Python has become more and more widely adopted over the past six years. 
In 2019, Python replaced Java as the most used language.
In 2021 and 2022, over half of the artifacts have Python code.
% We suspect that this is due to the growing number of papers related to machine learning. 
Java is still the second most widely used language, although its ratio has been decreasing year after year. 
The ratio of C/C++ is also decreasing.

The rising prominence of Python within the computer science community has driven this transformation. The expanding capabilities and user-friendly nature of Python libraries have simplified tasks that were previously accomplished using other programming languages. Consequently, possessing a fundamental understanding of Python has become increasingly essential for researchers.

\begin{figure}[h!]
\begin{center}
\includegraphics[width=0.45\textwidth]{images/figure_3.pdf}
\end{center}
\vspace{-5mm}
\caption{The number and ratio of artifacts with different programming languages.}
\label{progamminglanguage}
\end{figure}

\begin{findingbox}
Python has overtaken Java and become the most widely used language in SE artifacts and is getting more and more adoption, with its ratio increasing from 15.2\% in 2017 to 61.1\% in 2022. The ratios for Java and C/C++ are both decreasing. 
\end{findingbox}

\subsubsection{URL Location}
During the artifact collection process of our study, we observe that the location of the URL for an artifact in a paper makes a great difference in how easy it is for readers to notice its existence.
For instance, artifact URLs mentioned in the abstract or highlighted in the introduction section are easier to access than URLs given as textual implementation details.

Figure~\ref{fig:location}.(a) shows the distribution of artifact URL locations in different paper sections.\footnote{While some researchers multiply references to the URL, we count them in the first place we find it.}
We observe that 52.3\% of the papers with artifacts highlight the URL of artifacts in the abstract or introduction section.

The open-science policy such as 
% ICSE 2023
\cite{icse23policy} recommends authors provide artifacts in the section of Data Availability after the Conclusion section. 
In our collection, we find that only 5.0\% of all the URLs align with this recommendation in 2017-2021, which are provided with a separate section ``Data Availability'' after the conclusion. 
In 2022, however, this changes greatly. 11.4\% of the URLs are provided as recommended, demonstrating that the policy of ICSE 2023 and other similar recommendations have made a difference. 

40.9\% of the URLs are shown in the section that illustrates implementation details or other similar sections, which are more difficult to notice and search in our practice.

Figure~\ref{fig:location}.(b) shows the format that researchers choose to provide the URL. 
The distribution of URL formats is fairly even, with footnotes, references, and in-text citations each comprising around one-third of the total number of URLs: footnotes (33.5\%), references (28.2\%), and in-text citations (31.7\%).
4 (0.3\%) artifacts are provided with hyperlinks in the text.
Although there is no criterion for researchers to arrange their URL, we recommend not to provide the URL with a hyperlink such as ``click here'', for we find it is quite easy to miss the URL.


\begin{figure}
\begin{minipage}{0.49\linewidth}
  \centerline{\includegraphics[width=\textwidth]{images/figure_4a.pdf}}
  \centerline{(a)}
\end{minipage}
\hfill
\begin{minipage}{0.49\linewidth}
  \centerline{\includegraphics[width=\textwidth]{images/figure_4b.pdf}}
  \centerline{(b)}
\end{minipage}
\vfill
%\vspace{-5mm}
\caption{Distribution of artifact URL locations and formats provided in papers.}
\label{fig:location}
\end{figure}

\begin{findingbox}
{About half (52.3\%) of the publications with artifacts place the URL of artifacts in the abstract or introduction. Under the recommendation of ICSE 2023 and other conferences, 11.4\% of URLs in 2022 are provided in the section of Data Availability after the conclusion section.}
\end{findingbox}

\subsection{RQ2: Maintenance}
To answer RQ2, we analyze the validity of the URL and the last update time of an artifact.

\subsubsection{Link Rot}
Figure~\ref{invalidurls} illustrates the frequency of link rot in the SE research artifacts from 2017 to 2022. Overall, the proportion of artifacts suffering from the link rot issue increases over time, with an average of 9.4\%. Specifically, the proportions for these years are 29.8\%, 22.6\%, 5.2\%, 4.3\%, 1.8\%, and 4.8\%, respectively. 
Nearly one-third of artifacts provided in 2017 are unavailable due to link rot, around six times the ratio for 2022.

This finding is consistent with that observed by previous work (\cite{ChristopherTimperley2021}). 
In 2019,  \citeauthor{ChristopherTimperley2021} analyzed the URLs extracted from technical papers published in ICSE, FSE, ASE, and EMSE between 2014 and 2018. They found that 26.47\% of artifacts provided in 2014 were unavailable due to link rot, while the corresponding ratio for 2018 is 5.43\%.

We further analyze the unavailable artifacts in different types of storage websites. Figure~\ref{invalidurls-which} presents the results. We find that 32.6\% of artifacts originally stored on temporary drives (such as Dropbox and Google Drive) have become unavailable. 
Similarly, 11.8\% of artifacts on personal homepages are inaccessible. 
In contrast, the corresponding proportions of artifacts on GitHub and other artifact service platforms (such as Zenodo) are 6.4\% and 7.1\%. 
For the artifacts on GitHub, only when the researchers delete or hide the repository, does link rot happen. Updating does not matter, but for the artifacts on temporary drives, exceeding the sharing time limit or stopping sharing can contribute to link rot. The server changes, domain expiration, and personnel changes can all become the cause of link rot.

% The findings suggest researchers should not share their artifacts through personal homepages or temporary drives.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{images/figure_5.pdf}
% \vspace{-5mm}
\caption{The ratio of invalid URLs from 2017 to 2022.}
\label{invalidurls}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.45\textwidth]{images/figure_6.pdf}
% \vspace{-5mm}
\caption{The proportions of unavailable artifacts in different types of storage websites.}
\label{invalidurls-which}
\end{center}
\end{figure}

\begin{findingbox}
Overall, 9.4\% of the artifacts we collected are unavailable due to link rot. 
The proportion of link rot raises over time, from 4.8\% for publications in 2022 to 29.8\% in 2017. 
Link rot is more prevalent in temporary drives (32.6\%) and personal homepages (11.8\%) than on GitHub (6.4\%) and artifact service platforms (7.1\%). 
We suggest sharing artifacts through artifact service platforms.
\end{findingbox}

\subsubsection{The Latest Update Time}
Table~\ref{tabel:maintaince} shows the percentage of artifacts that were updated after their respective deadlines. 
For example, for the ICSE 2017 conference, 64.3\% of the artifacts were updated after the conference date.

More than 90\% of the artifacts were updated after the submission deadlines each year. 
However, the update rate drops after each subsequent milestone date. 
For instance, for ICSE 2022, 99.0\% of the artifacts were updated after the submission deadline, 91.1\% after the paper notification date, 77.2\% after the camera-ready deadline, and only 54.5\% after the conference date.

% We observe the update ratios of ISSTA are consistently higher than the other conferences, which may be attributed to ISSTA having fewer papers overall and any small changes being more significant.

When comparing the ratios of the same conference across different years, it is found that the percentage of artifacts updated after the conference date decreases over time. 
For example, in ICSE, 64.3\% of artifacts were updated in 2017, whereas 54.5\% were updated in 2022. A similar pattern is observed for the other three conferences. 
We speculate that older artifacts may receive regular attention and updates to fix bugs over time, while newer artifacts may not have received sufficient attention and encountered problems that require updates.

In general, the update rate of artifacts decreases over time for each conference. This could be due to projects losing maintenance or certain artifacts not requiring regular updates. However, for artifacts that implement tools, the lack of maintenance can make them increasingly difficult to use. It is challenging to measure researchers' level of care for their artifacts. We hope that researchers view artifacts as valuable assets that can be lost if not taken care of, rather than as mere appendages to papers that are forgotten over time.


\begin{table}[h!]
\normalsize
\caption{The maintenance situation of ASE, FSE, ICSE and ISSTA 2017-2022. Each number presents the ratio of artifacts that gets updated after each key time point.}
\begin{center}
\resizebox{0.49\textwidth}{!}{
%ASE
\begin{tabular}{llrrrr}
\toprule
\multirow{2}{*}{Conference}&\multirow{2}{*}{Year}&Submission&Paper&Camera-ready &Conference\\
&& deadline & notification & deadline &  time\\
\midrule
ASE & 2017 & 92.3\% & 88.5\% & 80.8\% & 76.9\% \\
& 2018 & 96.4\% & 89.3\% & 85.7\% & 78.6\% \\
& 2019 & 96.4\% & 85.7\% & 60.7\% & 53.6\% \\
& 2020 & 100.0\% & 95.6\% & 73.3\% & 62.2\% \\
& 2021 & 100.0\% & 97.8\% & 69.6\% & 52.2\% \\
& 2022 & 98.3\% & 93.2\% & 71.2\% & 55.9\% \\
& Average & 97.8\% & 92.7\% & 72.8\% & 61.2\% \\
\midrule
FSE & 2017 & 100.0\% & 92.0\% & 80.0\% & 68.0\% \\
& 2018 & 96.4\% & 89.3\% & 57.1\% & 46.4\% \\
& 2019 & 97.0\% & 90.9\% & 84.8\% & 78.8\% \\
& 2020 & 95.6\% & 95.6\% & 71.1\% & 60.0\% \\
& 2021 & 98.6\% & 92.9\% & 75.7\% & 47.1\% \\
& 2022 & 96.0\% & 92.0\% & 68.0\% & 46.0\% \\
& Average & 97.2\% & 92.4\% & 72.9\% & 55.4\% \\
\midrule
ICSE & 2017 & 100.0\% & 85.7\% & 85.7\% & 64.3\% \\
& 2018 & 97.1\% & 97.1\% & 85.3\% & 76.5\% \\
& 2019 & 100.0\% & 94.9\% & 84.6\% & 64.1\% \\
& 2020 & 98.1\% & 92.3\% & 73.1\% & 50.0\% \\
& 2021 & 96.7\% & 95.1\% & 78.7\% & 60.7\% \\
& 2022 & 99.0\% & 91.1\% & 77.2\% & 54.5\% \\
& Average & 98.3\% & 93.0\% & 79.1\% & 59.1\% \\
\midrule
ISSTA & 2017 & 100.0\% & 100.0\% & 100.0\% & 100.0\% \\
& 2018 & 100.0\% & 84.6\% & 84.6\% & 76.9\% \\
& 2019 & 90.9\% & 90.9\% & 81.8\% & 63.6\% \\
& 2020 & 95.8\% & 95.8\% & 83.3\% & 70.8\% \\
& 2021 & 96.4\% & 92.9\% & 82.1\% & 60.7\% \\
& 2022 & 100.0\% & 91.4\% & 77.1\% & 42.9\% \\
& Average & 97.4\% & 92.3\% & 82.1\% & 61.5\% \\
\bottomrule
\end{tabular}}
\end{center}
\label{tabel:maintaince}
\end{table}

\begin{findingbox}
Most (Over 90\%) artifacts need continuous maintenance and updating after submission.
The update ratio of earlier artifacts is higher than the newer ones.
\end{findingbox}

\subsection{RQ3: Popularity}
\label{sec:result:popularity}

% Clearly, the popularity of these arifacts is closely related to the subjects they study. No matter how perfect the artifact of an unpopular domain is, it is difficult to be more popular than a commonly used library, even if the latter's artifact may have all kinds of defects. We only focus on the characteristics of these most popular artifacts, and which domains are more popular is a complex issue, which is not our focus here.

The popularity of artifacts is closely tied to their impact, especially in the SE field. A more popular artifact has more chances to influence real-world applications and benefit people.
RQ3 focuses on the popularity of artifacts in the field of software engineering. 
We use the number of stars on GitHub as a measure to analyze the popularity of existing SE artifacts. 
Additionally, we study the characteristics of the most popular artifacts.

\subsubsection{Star situation}

\begin{table}[h!]
\caption{The distribution of star numbers of SE artifacts from 2017 to 2022. Each number presents the ratio of artifacts whose star numbers belong to the range in the first column.}
\begin{center}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lrrrrrrr}
\toprule
Year&0&1-5&6-10&11-20&21-50&51-100&100+\\
\midrule
2017 & 11.3\% & 42.3\% & 14.1\% & 14.1\% & 7.0\% & 9.9\% & 1.4\% \\
2018 & 13.6\% & 28.2\% & 12.6\% & 13.6\% & 17.5\% & 1.9\% & 12.6\% \\
2019 & 11.7\% & 29.7\% & 18.9\% & 17.1\% & 14.4\% & 1.8\% & 6.3\% \\
2020 & 15.1\% & 39.2\% & 18.1\% & 11.4\% & 10.2\% & 4.2\% & 1.8\% \\
2021 & 12.2\% & 37.6\% & 17.1\% & 14.6\% & 11.2\% & 5.9\% & 1.5\% \\
2022 & 13.5\% & 31.8\% & 19.2\% & 18.8\% & 13.9\% & 0.4\% & 2.4\% \\
\midrule
Average & 13.1\% & 34.6\% & 17.3\% & 15.3\% & 12.5\% & 3.4\% & 3.7\% \\
\bottomrule
\end{tabular}}
\end{center}
\label{tabel:star}
\end{table}

Table~\ref{tabel:star} shows the distribution of the star numbers of the SE artifacts from 2017 to 2022. 

In general, the number of artifact stars is generally small. While 3.7\% of artifacts have over 100 stars, 65.0\% have equal or less than 10 stars. 13.1\% of the artifacts even do not have any stars at all. 
Only eight artifacts have more than 300 stars.
We can observe more clearly that the star numbers concentrate on a low level, indicating the overall low popularity of the SE artifacts.

Furthermore, one might expect a positive correlation between the creation date of an artifact and the number of stars it accumulates. However, our analysis does not reveal a clear relationship between star counts and time. 
To some extent, the 2022 data is indeed more concentrated in the lower number range than the 2017 data, but the data for other years does not exhibit a consistent pattern.

\begin{findingbox}
In general, the popularity of the SE artifacts on GitHub is low, with only 3.7\% of artifacts having over 100 stars and 65.0\% having equal or less than 10 stars. Star numbers and time did not show a clear correlation.
\end{findingbox}

\subsubsection{Characteristics}
The low popularity of existing SE artifacts motivates us to characterize the top-starred artifacts to provide implications for improving future artifacts and their popularity. 

\revise{
To this end, we consider artifacts with more than 100 stars as top-starred ones. 
By applying this criterion, we identify 33 top-starred artifacts in total.
}
We compare them with widely adopted criteria in the research community (\cite{acmguidelines}), and discuss how these top-starred artifacts meet the criteria.

\revise{
According to our analysis, all 33 top-starred artifacts are documented and possess comprehensive documentation, covering the introduction, usage, and examples. 
28 of these top artifacts are accompanied by licenses. All the top-starred artifacts are still maintained one year after the publication year of their papers.
It is worth noting that all the top-starred artifacts contain executable code and have a significant impact on real-world applications.
Notably, 15 of these artifacts have surpassed 50 forks, while 17 have accumulated more than 50 issues.
}

As mentioned above, We only focus on the characteristics of these most popular artifacts, and their research objects are beyond the scope of our research.

\begin{findingbox}
\revise{
Overall, all 33 top-starred artifacts possess comprehensive documentation and are still maintained one year after their publication.
The top-starred artifacts bring a significant impact on real-world applications.
}
\end{findingbox}

\revise{
Note that the popularity of artifacts cannot be determined solely based on the number of stars. 
Other metrics, such as issues and forks, could also be taken into consideration. 
To enhance the comprehensiveness of our popularity analysis, we leverage the GitHub API to explore these two metrics for the relevant GitHub artifacts as an additional analytical approach.
We observe that 45\% of GitHub artifacts have no issues, while 80\% have less than ten issues. In terms of fork numbers, nearly 90\% of artifacts have fewer than ten forks. Moreover, the distribution of issues and forks does not exhibit significant differences among artifacts from different years.
Overall, the distribution of these metrics for artifacts closely resembles that of stars. 
Because stars are more prevalent across a larger number of repositories, our analysis primarily focuses on the star number.
}

\subsection{RQ4: Quality}
\label{sec:result:quality}
The last research question characterizes the quality of artifacts from two aspects: the content of documentation and the circumstances of code smell. 

\subsubsection{Documentation}
\label{sec:result:quality:document}
This section explores the content of the documentation of the artifacts. 

The results are shown in Figure~\ref{fig:documentation}.
The completeness of the README went worse, from 50.0\% in 2017 to 43.6\% in 2019. Then it is slowly recovering, finally at 56.4\% in 2022 and with a total average of 49.8\%. 
The ratios of Structure, Usability, and Example are 27.9\%, 60.8\%, and 26.2\% on average. 
The case of Certificate is getting better, from only 28.6\% in 2017 to 47.5\% in 2022. 
The ratio of Contact shows a noticeable decline in 2022, accounting for only 27.7\% in that year.
This may be because it is the newest and not too many issues have appeared.

In addition, we have some interesting findings. The artifacts often meet Completeness and Usability together. 
97.5\% of the artifacts that meet Example at the same time meet Usability altogether. 
The artifacts meeting Structure is often an artifact of a survey, an empirical study, or a data set.

\begin{findingbox}
In general, artifact documentation quality is fair and has not changed much in recent years. Overall, researchers do better in Completeness, Usability, Certificate, and Contact than in the other two criteria, Structure, and Example. There is still room for improvement on all criteria.
\end{findingbox}


\begin{figure*}[h!]
\begin{center}
\includegraphics[width=0.95\textwidth]{images/figure_9.pdf}
\end{center}
\vspace{-5mm}
\caption{The documentation situation of ICSE artifacts.}
\label{fig:documentation}
\end{figure*}

\subsubsection{Code Smell}
This section explores the smells of the code researchers write in their artifacts.
We focus on Python and Java code because they are covered by the majority of the artifacts.

% Note that we only care about the smells of the code written by researchers, other than the code from existing datasets or libraries written by other developers (more details in Section~\ref{sec:methodology}).

\textbf{Python}. We detect the code written in Python by \cite{pylint}. 
Pylint produces code smell results for 268 Python artifacts within a limited time (1 minute), and provides three types of code smells\footnote{While Pylint also provides information in three other categories, including ``Fatal'', ``Error'', and ``Information'', these three are not considered as indicators of a code smell. This is because code smells indicate potentially flawed or suboptimal coding practices instead of bugs or other information.}: 
(1) Convention: the code violates recommended coding conventions; 
(2) Refactor: the code needs effort in refactoring;
(3) Warning: the code contains issues that developers may need to fix, but the issues are not fatal enough to terminate the running of the code.
The detailed content for each type of alert message, explanation, and specific examples can be found in the documentation of \cite{pylintmessageoverview}.

% 28 + 35 + 40 + 21 + 26 + 45
\textbf{Java}.
We use \cite{pmd} to detect the smells in Java code.
PMD successfully runs on all 195 Java artifacts, and we use them as our analysis subjects.
Different from Pylint, PMD provides more diverse alert messages, including
(1) Code style: the code violates a specific coding style;
(2) Documentation: the code needs effort in code documentation;
(3) Design: the code contains design issues;
(4) Best Practices: the code violates generally accepted best practices;
(5) Error Prone: the code contains constructs that are either broken, extremely confusing, or prone to runtime errors;
(6) Performance: the code contains suboptimal code;
(7) Multithreading: the code contains issues when dealing with multiple threads of execution;
(8) Security: the code contains potential security flaws\footnote{Please refer to \url{https://pmd.github.io/latest/pmd_rules_java.html} for more details of each message.}.


Figure~\ref{fig:codesmell}.(a) and (b) show the distribution for each type of alert message in Python and Java artifacts.
For Python, the ratio of Convention messages about coding convention violations is the most common, which accounts for 52.3\%. 
There are also 38.7\% warning messages and 9.0\% refactoring alerts. 
The most common smell for Java is code style, similar to convention violations.
These issues may affect the artifacts' readability, maintainability, and usability. It is unsurprising that these issues exist because researchers are often not well-trained developers.
However, poor code styles can make the code hard to understand, maintain, reuse, and even contain potential bugs. While poor code style does not cause major problems in most cases, so many small flaws combined in a single artifact can overwhelm valuable insights in the code, making the paper difficult to understand and reuse. Therefore, code style is also an important part of a paper and should be considered when evaluating papers.

\begin{figure}
\begin{minipage}{0.48\linewidth}
  \centerline{\includegraphics[width=\textwidth]{images/figure_7b.pdf}}
  
  \centerline{(a)}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
  \centerline{\includegraphics[width=\textwidth]{images/figure_7a.pdf}}
  \centerline{(b)}
\end{minipage}
\vfill
%\vspace{-5mm}
\caption{Ratio of different types of Python (a) and Java (b) messages from 2017 to 2022.}
\label{fig:codesmell}
\end{figure}

We further dive deep into these alert messages and check their prevalence and specific contents.
Column ``Prevalence'' in Table~\ref{codequalitycount} shows the number of artifacts with the corresponding type of alert messages against the total number of artifacts.
We observe that all the alert messages are surprisingly prevalent in the artifacts.
For example, 254 out of the 268 (98.5\%) artifacts in Python are recommended to refactor their code.  
The average prevalence ratio (the first number divided by the second number in Column ``Prevalence'') of the alert messages is 96.0\% for Python and 98.3\% for Java.

Column ``Name'' and Column ``Explanation'' in Table~\ref{codequalitycount} represent the top three most common alert messages under each message category and their explanation.
We hope that these results could shed light on issues to avoid when researchers wish to improve the quality of their code when preparing artifacts (more details in Section~\ref{sec:Discussion}).

\begin{table*}[h!]
\normalsize
\caption{The top three most common alert messages under each smell category for Python (top three rows) and Java (bottom seven rows).}
\begin{center}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{lrllr}
\toprule
Type&Prevalence&Name&Explanation&Pct.(\%)\\

\midrule
\multirow{3}*{Convention} & \multirow{3}*{260/268} & invalid-name&Code violates naming rules for variables. & 23.4 \\
 & & line-too-long&Code has a line longer than 100 characters. & 19.9 \\
 & & missing-function-docstring&Code contains a function or method without a docstring. & 19.3 \\
\midrule
\multirow{3}*{Warning} & \multirow{3}*{258/268} & bad-indentation&Code has incorrect indentation. & 58.4 \\
 & &unused-import&Code imports unused modules or variables. & 6.5 \\
 & & redefined-outer-name &Variable in inner scope shares the same name as one in outer scope. & 5.0 \\
\midrule
\multirow{3}*{Refactor} & \multirow{3}*{254/268} & consider-using-with & A resource-allocating assignment may be replaced by a ``with'' block. & 13.1 \\
 & & too-many-locals&Function or method has over 15 local variables. & 10.9 \\
 & & no-else-return&Unnecessary "else" block with a "return" statement. & 9.9 \\

\bottomrule

\toprule

\multirow{3}*{Best Practices} & \multirow{3}*{144/144} & SystemPrintln & Code can use a logger instead of System.out.print references. & 15.8 \\
 &  & LooseCoupling & Code has excessive coupling implementation types. & 8.7 \\
 &  & UnusedAssignment & Code has unused variable assignments. & 8.7 \\
\midrule
\multirow{3}*{Code Style} & \multirow{3}*{144/144} & LocalVariableCouldBeFinal & Local variable assigned only once can be declared final. & 26.5 \\
 &  & MethodArgumentCouldBeFinal & Method argument never reassigned can be declared final. & 22.2 \\
 &  & ShortVariable & Fields, variables, or parameters have very short names. & 11.5 \\
\midrule
\multirow{3}*{Design} & \multirow{3}*{144/144} & LawOfDemeter & Code violates the Law of Demeter. & 29.3 \\
 &  & CyclomaticComplexity & Methods/classes should be broken down into smaller components. & 8.6 \\
 &  & CognitiveComplexity & Methods are too complex. & 6.7 \\
\midrule
\multirow{3}*{Documentation} & \multirow{3}*{144/144} & CommentSize & Comments exceed specified size limits. & 49.8 \\
 &  & CommentRequired & Code needs more comments. & 48.7 \\
 &  & UncommentedEmptyMethodBody & Empty method body without comments. & 1.2 \\
\midrule
\multirow{3}*{Error Prone} & \multirow{3}*{140/144} & AvoidLiteralsInIfCondition & Hard-coded literals used in conditional statements. & 22.1 \\
 &  & AvoidDuplicateLiterals & Duplicate String literals should be declared as constant fields. & 10.7 \\
 &  & DetachedTestCase & Test case method should be detached. & 9.0 \\
\midrule
\multirow{3}*{Multithreading} & \multirow{3}*{134/144} & DoNotUseThreads & Code violates the J2EE specification by using threads. & 34.9 \\
 &  & UseConcurrentHashMap & Code can use the Map designed for multi-threaded access in Java5. & 32.4 \\
 &  & AvoidSynchronizedAtMethodLevel & Method-level synchronization can cause problems with new code. & 21.4 \\
\midrule
\multirow{3}*{Performance} & \multirow{3}*{141/144} & AvoidInstantiatingObjectsInLoops & New objects created within loops should be checked and reused. & 37.8 \\
 &  & RedundantFieldInitializer & Explicit initialization of default values that will be initialized by Java. & 16.7 \\
 &  & ConsecutiveAppendsShouldReuse & Consecutive calls to StringBuffer/StringBuilder appends should be chained. & 8.9 \\

\bottomrule
\end{tabular}}
\label{codequalitycount}
\end{center}
\end{table*}


\begin{findingbox}
Code smells are prevalent in the artifacts.
On average, code smell alert messages appear in 96.0\% of the Python projects and 98.3\% of the Java projects.
The majority of the code smell alert messages are related to code convention violations.
\end{findingbox}


\section{Discussion}
\label{sec:Discussion}

In this section, we present our suggestions and discuss the threats to validity.

\subsection{Suggestion}
Based on our findings, we discuss insights on the status and trends of SE artifacts and provide further suggestions.

\subsubsection{Common Practices}

Regarding \textbf{storage websites} of artifacts, though SE conferences (\cite{icse21policy,icse22policy}) have exploited recommend archiving platforms like Zenodo over version control systems like GitHub, the majority (64.2\% in 2022) of publications choose GitHub for their artifacts.
Because GitHub is easier to maintain and allows for updating the artifacts, we believe GitHub will still be one of the most trending artifact storage websites in the near future.
Additionally, GitHub has a similar link rot rate to Zenodo, which shows that artifacts stored on GitHub can be maintained for a long time.
Besides, most (over 90\%) artifacts have the update requirement after the submission,  indicating that version control systems like GitHub can satisfy the requirement better than archiving platforms like Zenodo. 
Therefore, we suggest that conferences should not blanket exclude version control systems like GitHub, but instead provide guidance on choosing the appropriate platform for specific artifacts.

Moreover, we observe a rapid increase in the use of Zenodo (0.0\% in 2017 to 16.0\% in 2022), which is more suitable for artifacts that do not need to be updated over time, such as datasets. The adoption ratio of Zenodo will likely increase further given its recommendation by conferences as well as its advantages for long-term preservation. We suggest SE researcher choose Zenodo for suitable artifacts.

In terms of \textbf{programming language}, the use of Python has increased from 15.2\% in 2017 to 61.1\% in 2022, surpassing Java. The adoption of Java and C/C++ has decreased over the past six years. We expect this trend to continue going forward.
While quality metrics (e.g. code smells) and detection tools are mature for Java, those for Python are still lacking. 
Given the majority of artifacts now use Python, the SE research community can define coding conventions and specific rules for Python code in artifacts to improve readability and standardization. 
Providing guidance and examination tools for Python artifact code would also enhance quality and reusability.

As for the \textbf{URL location}, we find that 40.9\% artifact URLs are hidden in the middle of the paper and are easily overlooked.
The community has recommended unifying the artifact URL location in the ``Data Availability'' section after the conclusion. 
Although the compliance rate with this rule is still low, there has been a rapid increase in recent years. Unifying artifact URL locations makes it easier to find and access artifacts, increasing their impact. 
We suggest that more publications follow this rule and prominently display artifact URLs in papers, as the increasing importance of artifacts.

% we recommend avoiding using temporary drives and self-built homepages, according to the observation of RQ2 and the guidelines of FSE 2021  \cite{fse21guidelines} and ICSE 2023 \cite{icse23policy}. These two types of storage websites can easily cause link rot, making artifacts unavailable. In addition, the guidelines suggest researchers use preserved digital repositories (such as Zenodo) to archive their artifacts.

% For the URL location, we recommend the research community to unify the artifact URL location to make it easy for others to find the URL.
% ICSE 2023 \cite{icse23policy} suggest authors put the artifact URL after the Conclusion section. We observe that only 8.8\% of artifacts align with this rule between 2017 and 2021. In contrast, 52.6\% of papers provide the artifact URL in the abstract and introduction. However, it is a delight that 20.9\% of artifacts follow this rule in 2022.

% We recommend avoiding providing artifact URLs in the hyperlink format.
% According to RQ1, there are still 5 artifacts provide hyperlinks as URLs of artifacts, which is hard for readers to find. It's harmful to the smooth usage of the artifact and should be avoided in the future.

\subsubsection{Maintenance}


Regarding artifact availability, the \textbf{link rot} rate increased over the years, with up to around one-third of artifacts inaccessible in 2017. To ensure the long-term accessibility of SE artifacts, the SE community should give additional consideration to artifacts' longevity when reviewing papers, especially for artifacts stored on temporary drives and personal websites that exhibit significantly higher link rot rates than those on GitHub and Zenodo.

For the \textbf{last update time}, most artifacts need continuous updating after submission, highlighting the high updating needs and propensity to become outdated of SE research artifacts. 
Earlier artifacts have a higher update rate. 
We believe that if the community and researchers want to ensure artifacts remain useful and reproducible over time, only one artifact examination before conferences is insufficient.
Given their tendency to become obsolete quickly, regular re-examination is worthwhile for valuable artifacts to keep them up-to-date, effective, and reproducible in the long term.


% For the Link rot, recovering is much more difficult than maintenance. As we observe and mentioned in RQ2.1, avoiding deleting the repository for artifact on GitHub can help. If researchers have to replace the artifact to another place, we suggest still leaving a README file explaining the situation and the new URL. Link rot happens more on Personal homepage and Temporary drive. Avoid using them as just mentioned in the suggestion for common practice.

% For the last update time, we recommend coming back to the artifact regularly and checking the possible messages. If there is nothing to change, adding a sentence like ``The repository is still under maintenance at 2020.10'' or just refreshing the last update time are both suitable. Avoid forgetting the artifact and never checking it again as papers are hired and conferences are held.

\subsubsection{Popularity}
% For Star numbers, it is difficult to earn lots of stars for an artifact, but this does not mean the artifacts are not important. We suggest taking artifacts seriously.


% For Characteristics, we suggest that artifacts align with the top-starred practices. As reported in a previous study~\cite{ChristopherTimperley2021}, less than half of the respondents have experience with artifact (re-)use, which illustrates the pessimistic popularity situation of artifacts. RQ2 also summarizes the low popularity of artifacts, with 72.2\% of artifacts having fewer than 10 stars and 16.8\% of artifacts having no star. The low level of star distribution of artifacts aligns with the few experience using artifacts. To realize the best reproduced and replicated potential of the artifacts, we suggest that artifacts align with the top-starred practices.

Regarding \textbf{star numbers}, most GitHub artifacts receive limited attention, with 65.0\% attracting no more than 10 stars. 
Though artifact star counts are not an accurate measure of popularity, they indicate that most software engineering artifacts lack real-world adoption and impact.
Artifacts may struggle to gain traction because most target niche audiences. 
Even for intended audiences, less than half of respondents report experience reusing artifacts (\cite{ChristopherTimperley2021}).
However, we believe that some prototyped artifacts could have great potential to influence real-world applications and facilitate people's lives if properly disseminated. 
Such artifacts should be viewed not just as paper attachments, but as vital contributions of SE research, advancing the practical implications of software engineering.

We believe that conferences can increase the usefulness and impact of SE artifacts by incorporating \textbf{characteristics} of top-starred artifacts into their evaluation criteria and recommendations, including providing detailed documentation and easy install packages, as well as keeping maintenance.

\subsubsection{Quality}

In terms of \textbf{documentation}, artifact documentation often lacks descriptions of file structure and usage examples, which are vital for most artifacts. 
Describing an artifact's file structure helps users quickly comprehend its composition and working mechanism. 
Usage examples assist users in verifying artifacts that provide tools work properly.
% Besides, 3.2\% of artifacts still lack documentation entirely, severely hampering artifact reproducibility.
Therefore, We suggest conferences remind researchers to include file structure descriptions and usage examples for suitable artifacts, achieving better documentation quality.

For code quality, we perform \textbf{code smell} tests on Python and Java artifacts and find that over 96\% of artifacts incur alerts. 
Most alerts relate to code convention, not functionality.
As function correctness instead of code convention matters most for code in artifacts, we conclude that the commonly-used metrics for general SE projects, code smells, are unsuitable for artifacts. 
Therefore, we suggest more research on better code quality metrics for artifacts in the SE field, especially for Python.

% For Code quality, it is not considered as important for artifact evaluation purpose, as introduced in previous work \cite{hermannCommunityExpectationsArtifacts2020}. However, if researchers want to provide an artifact with high code quality, we recommend focusing more on the recommended coding convention of Python and the coding style of Java, as RQ4 shows the proportion of alert messages.


\revise{
\subsubsection{Summary}

Based on previous analysis, we summarize suggestions for different stakeholders.

\textbf{For organizers of SE publications:}

(1) Enhance Artifact Preparation Guidance.
Provide comprehensive guidance and detailed assessing criteria for artifact preparation, encompassing aspects such as storage platform selection, document quality enhancement, and subsequent maintenance strategies.

(2) Promote Inclusive Artifact Guidance.
Conferences should avoid blanket exclusions and guide authors in selecting the right platform for their artifacts. 
For static datasets, Zenodo is recommended for archiving, while GitHub is preferred for artifacts involving iterative code updates, with a release version as an archive. 
Conference organizers can provide detailed instructions on different platform features to cater to diverse needs.

(3) Unify the artifact URL in a prominent location. 
As the importance of artifacts becomes increasingly recognized, artifact URLs in papers should be highlighted to facilitate reader access.
Conference organizers can provide a unified recommended position of artifact URLs in the guidance or integrate the URLs into the publication metadata.

(4) Consider artifact longevity during the review process.
Conference organizers should discourage the use of temporary drives or personal websites to host artifacts and consider the long-term validity of artifacts during the review process to minimize the risk of link rot.


(5) Provide high-quality artifact examples.
Offering exemplary artifacts of various types can help authors in producing higher-quality artifacts. For instance, the guidance may present highly acclaimed artifacts from previous years' publications and utilize their characteristics as recommended and evaluative criteria, such as providing easy installation packages, test cases, and comprehensive documents.

(6) Promote real-world adoption and impact.
Conference organizers can encourage researchers to integrate their artifacts into practical application development and promote their potential impact.
We recommend extending the evaluation and recognition of artifacts beyond publications through regular evaluations and giving recognition to those artifacts that demonstrate significant impact.

\textbf{For researchers.}

(1) Emphasize the contribution of artifacts.
To enhance the replication of papers, researchers should strive to provide artifacts for their papers whenever possible and prominently highlight them as a significant contribution to papers.

(2) Choose a suitable storage platform for artifacts.
Researchers should consider factors such as maintenance frequency, long-term storage link availability, sharing options, and data size when selecting a storage platform for artifacts. 
For large static datasets, Zenodo is a recommended choice, while GitHub is suitable for small codebases that require regular updates and maintenance. 
We recommend minimizing the use of personal websites and temporary data drives, which are more prone to link rot.
Moreover, we suggest researchers provide an archived version of the artifacts as a snapshot, regardless of the selected platform.

(3) Enhance artifact quality.
Researchers should improve the quality of artifacts to facilitate the reproducibility of their paper's results by other users. Enhancing artifact quality involves attention to various details, such as comprehensive documentation, clear file structure explanations, simple installation scripts and examples, author contact information, and improved code readability.

(4) Maintain artifacts regularly.
To ensure the long-term usefulness and impact of artifacts, researchers should regularly maintain them. Maintenance tasks include promptly responding to user inquiries, updating dependencies, addressing software versioning issues, and incorporating new features or improvements.

\textbf{For software engineering community.}

(1) Embrace open science practices.
The community should continue supporting and promoting the sharing of open-source artifacts. 
This will foster transparency, reproducibility, and collaboration among researchers.

(2) Promote tools and technologies for artifact management. 
Addressing issues such as link rot and ensuring the enduring availability of artifacts stored outside commonly used platforms can be facilitated by developing tools or leveraging existing technologies like the Wayback Machine and robust links.

(3) Conduct further research on artifact quality metrics. 
The SE community can prioritize research and development of metrics and automated examination approaches specifically tailored to different programming languages and artifact types.
Specifically, the community can offer further guidance and examination tools for Python artifacts, given that Python is the most widely used programming language in current software engineering artifacts.

% Summary, do not delete
% In general, as the ratio of software engineering publications containing artifacts has risen from 60\% in 2017 to 81\% in 2022, the value of open research artifacts has become accepted wisdom within the software engineering community. 
% This increased prevalence of artifacts aims to enrich SE research evidence and reproducibility. 
% The trend is expected to continue, with an ever larger proportion of SE papers providing artifacts. 
% However, not all artifacts effectively fulfill their purpose as part of the research. 
% We find that 9 artifacts contain only the paper title and 3.4\% -- 19.4\% of artifacts become inaccessible over time due to link rot, seriously harming reproducibility. 
% As such, the research community's focus should shift from merely having artifacts to having high-utility artifacts that genuinely help advance research. 
% SE researchers and the community should make efforts to maximize artifacts' usefulness for future work.
}

\subsection{Threats to validity}
\noindent \textbf{Manually check.}
We carry out the empirical study with many manual checks.
Therefore, there are some potential threats to validity.
Multiple checkers are involved in the manual checking process and there is a risk that their judgments may not be consistent.
Besides, the manual checking process could be influenced by biases on the part of the checkers, such as confirmation bias or selection bias. These biases could affect the results of the study and reduce its validity.
Our checkers communicate with each other as much as possible, eliminating subjective differences between different checkers. However, this may still affect.

\noindent \textbf{Selection of storage website.}
We chose artifacts in GitHub to examine their popularity. However, the star number is a  GitHub-specific metric and may not apply to other platforms like Zenodo. 
We also measured artifacts in other platforms that provide star numbers and found similar observations.

\section{Related Work}
\label{sec:Related Work}

In this section, we introduce existing work on community expectations of artifacts. Then, we summarize the work related to the replicability of software engineering.

\subsection{Community Expectations of Artifacts}

Artifact evaluation attracts great attention in software engineering. 
Many previous work propose the recommendations and expectations of artifacts (\cite{hermannCommunityExpectationsArtifacts2020, ChristopherTimperley2021, fanWhatMakesPopular2021, liuReproducibilityReplicabilityDeep2022, di2017software}). Also, some guidelines have been proposed to describe the expected practice of the publications (\cite{fse21guidelines, acmguidelines, icse23policy,vidoni2021software}).

In 2013, 
% Krishnamurthi et al.
\cite{krishnamurthi2013artifact} proposed that software and other digital artifacts were amongst the most valuable contributions of computer science but conferences treated these mostly as second-class artifacts. As a result, they highlighted the importance of artifacts and argued for elevating these other artifacts by making them part of the evaluation process for papers. 

% Hermann et al.
\cite{hermannCommunityExpectationsArtifacts2020} provided an overview of the current perception of artifact evaluation and the community expectations toward artifacts. They conducted a survey among the artifact evaluation committees (AEC) members and analysed the purpose and community expectation of the artifact evaluation. In details, they extracted the key information from the response of AEC members and gained the expectations from reviewers and users perspectives. 


% Timperley et al.~
\cite{ChristopherTimperley2021} conducted an empirical study to understand how artifacts are created, shared, used, and reviewed by mixed methods. They analyzed all research-track papers published at four software engineering venues (ASE, EMSE, FSE, and ICSE) between 2014 and 2018 to determine the prevalence and availability of artifacts, and conducted a survey of 153 authors to identify the challenges of creating, sharing, using, and reviewing artifacts. Based on their finding, they derived several recommendations for different stakeholders in research. Their study is similar to ours to some extend. Our results can better reflect the current status and trends of artifacts because the data we used is from 2017 to 2022. We make many comparison with their findings in our work.

We also compare our findings with the guidelines of 
% FSE
\cite{fse21guidelines} and 
% ICSE
\cite{icse23policy}, and the 
% ACM guidelines 
\cite{acmguidelines} guidelines, which describe the expected characteristics of artifacts of publications in the above sections.


\subsection{Replicability in Software Engineering}

Replicability has become an important concern in software engineering research (\cite{flittner2018survey, saucez2019evaluating}), and ongoing work focuses on the quality, reliability, and trustworthiness of software engineering research results through the development and application of effective replicability techniques.

% Liu et al.~
\citeauthor{liuReproducibilityReplicabilityDeep2022} 
conducted a literature review on 147 DL studies published in 20 SE venues and 20 AI venues to investigate these issues and re-ran four representative DL models in SE to investigate important factors that may strongly affect the reproducibility and replicability of a study. They concluded that it is urgent for the SE community to provide a long-lasting link to a high-quality reproduction package, enhance DL-based solution stability and convergence, and avoid performance sensitivity on different sampled data, which is proved by our work another time.

% Anchundia et al.
\citeauthor{8951162} aim to identify tools that maximize reproducibility in software engineering experiments and how they are applied and performed a systematic mapping study and complementary strategies to analyze replication from communication concern, knowledge management concern, and motivation concern. They concluded that reproducibility is mostly relegated to internal replication, at which time and costs can be assumed within research groups and a focus on new alternatives should be considered to broaden replication.

Our work confirms these results and puts forward recommendations on how to better prepare artifacts, which will help improve replicability.


% our work's highlight
\section{Conclusion and Future Work}
\label{sec:Conclusion}

% conclusion
\revise{
We conduct an empirical study to understand the current status and trends of research artifacts in SE publications.
We conduct a dataset with 2,196 papers and corresponding 1,487 artifacts for analysis.
Based on the dataset, We investigate the common practices, maintenance, popularity, and quality. 
We observe an increase in the number of papers providing artifacts in SE venues.
The most commonly used storage platform is still GitHub, while the employment of Zenodo rapidly grows.
Over 90\% of artifacts would be updated after the submission.
At the same time, 65.0\% of artifacts have less than 10 stars and the code smell alert messages appear in 96.0\% of the Python projects and 98.3\% of the Java projects.
Moreover, we provide the discussion on the overall status of SE artifacts and offer suggestions to different stakeholders.
We hope our data and empirical results can support further study on the research artifacts of the SE community. 
}

\revise{
\subsection{Future Work}

\noindent \textbf{More venues.}
To capture the latest status and trends in the SE community, we study publications of four top-tier SE venues according to the CS Ranking. 
However, we could uncover more interesting findings if we expand our methodology and include a broader range of SE venues, including journals and more popular SE conferences with various requirements for artifacts.

Note that the annotation work is labor-intensive, as it entails manually searching for the artifact URLs for each paper and manually accessing, downloading, and analyzing them. As a starting point, we have developed a website, CS-Artifacts\footnote{http://ra.bdware.cn}, to showcase our annotated papers and their corresponding artifact data. We aim to gradually expand the coverage of venues on this website in the future.
}


\section{Data Availability}
\label{Data Availability}

We make our data, scripts, and results publicly available at \url{https://github.com/morgen52/SE-artifact}.


